Data Valuation for Vertical Federated Learning: A Model-free and Privacy-preserving Method

Vertical Federated learning (VFL) is a promising paradigm for predictive analytics, empowering an organization (i.e., task party) to enhance its predictive models through collaborations with multiple data suppliers (i.e., data parties) in a decentralized and privacy-preserving way. Despite the fast-growing interest in VFL, the lack of effective and secure tools for assessing the value of data owned by data parties hinders the application of VFL in business contexts. In response, we propose FedValue, a privacy-preserving, task-specific but model-free data valuation method for VFL, which consists of a data valuation metric and a federated computation method. Specifically, we first introduce a novel data valuation metric, namely MShapley-CMI. The metric evaluates a data party's contribution to a predictive analytics task without the need of executing a machine learning model, making it well-suited for real-world applications of VFL. Next, we develop an innovative federated computation method that calculates the MShapley-CMI value for each data party in a privacy-preserving manner. Extensive experiments conducted on six public datasets validate the efficacy of FedValue for data valuation in the context of VFL. In addition, we illustrate the practical utility of FedValue with a case study involving federated movie recommendations.

==> VFLValue AIJ/discussion.tex <==
%\section{Discussion}

%\textbf{Data Valuation considering Party Joining Order}. In multi-party VHL, in fact the party joining order may impact their data values. In general, if there are already more parties in the federation, then a new party joining the federation will receive lower data values.

\section{Conclusion}
In this paper, we proposed a novel data valuation method  named \emph{FedValue} for VFL. Specifically, we first designed Shapley-CMI, a task-specific but model-free data valuation metric based on information theory and game theory. We then proposed a new dual-server-aided mechanism to calculate Shapley-CMI in a federated manner and ensure that no party's private data will be leaked during the computation process. %In particular, we design a new dual-server-aided PSI mechanism to compute the size of different parties' intersection set in a privacy-preserving manner.
Finally, we accelerated FedValue with some practical computation techniques. Extensive experiments on six real-life datasets verified the effectiveness of FedValue.

As a pilot study on model-free data valuation of VFL, our study may inspire a series of future work as follows: (i) While we propose some practical acceleration methods for FedValue, its performance on different datasets varies obviously, calling for further research on the efficiency issue; (ii) Our work provides a prototype design for VFL data valuation, while implementing it in reality may face other challenges. For example, some parties may encounter communication problems and fail to upload their information --- how to deal with such connection losses needs careful design. 

\section*{Acknowledgement} 
We note that the authors contribute equally and are listed in alphabetical order. This study was partially funded by the National Natural Science Foundation of China under grant Nos. 72071125, 72031001 and 61972008.

==> VFLValue AIJ/experiment.tex <==

\section{Experiments}
\label{sec:experiment}

\begin{table}[t!]
    \small
    \centering
	\footnotesize
	\caption{Dataset Statistics}
	\label{tbl:dataset_stat}
	\vspace{-1em}
	\begin{tabular}{@{}lccc@{}}
		\toprule
		& \textit{\#features} & \textit{\#labels} & \textit{\#samples} \\ \midrule
		\textit{Wine} & 13 & 3 & 178 \\
		\textit{Parkinsons} & 22 & 2 & 195 \\
		\textit{Spect} & 22 & 2 & 267 \\
		\textit{Breast} & 30 & 2 & 569 \\
		\textit{Music} & 57 & 10 & 1000\\
		\textit{Credit} & 23 & 2 & 30000 \\
		\bottomrule
	\end{tabular}
\vspace{-1em}
\end{table}
We conduct extensive experiments to verify FedValue with six real-world datasets, including \textit{Wine} \cite{aeberhard1994comparative}, \textit{Parkinsons} \cite{little2007exploiting}, \textit{Spect} \cite{kurgan2001knowledge}, \textit{Breast} \cite{mangasarian1995breast}, \textit{Music}\footnote{\url{https://www.kaggle.com/andradaolteanu/gtzan-dataset-music-genre-classification}}, and \textit{Credit} \cite{yeh2009comparisons}. The dataset statistics are summarized in Table \ref{tbl:dataset_stat}. %The feature number of our selected datasets range from 11 to 30, aiming to verify the effectiveness of our mechanism in the learning tasks of different scales.
We discretize the continuous features of the datasets into five equal-width-bin categorical features to facilitate CMI computation following the literature \cite{Brown2012}. Next, we successively evaluate the effectiveness of FedValue, its computational efficiency, and the effects of practical computational techniques.

%We conduct extensive experiments to verify FedValue from two aspects:

%1) \textbf{Method Effectiveness}. Can Shapley-CMI effectively valuate the data parties' contribution to a VFL task given the task party? Can FedValue precisely compute Shapley-CMI for each party in a federated paradigm? % Specifically, we would compare Shapley-CMI to widely-used data valuation measures like SHAP \cite{Lundberg2017} to test whether Shapley-CMI can achieve better valuation quality on a variety of real-life datasets.

%2) \textbf{Practical Technique Performance}. Can the approximation results be close to the Shapley-CMI calculated in the original way?

%2) \textbf{Computation Efficiency}. How long does FedValue take to compute Shapley-CMI in various practical scenarios?%To answer this question, we will run a large number of experiments by varying the number of parties, features, etc. to see how the computation efficiency changes. We will also check how the approximation methods can reduce the computation time.



%It is worth noting that, Q1 is hard to , as there is no ground truth for the data values. In literature, most studies focus only on validating it is common that only case studies are illustrated to qualitatively demonstrate the effectiveness of data valuation \cite{Wang2019}.

%\subsection{Datasets}



%\subsubsection{Parameters}
%\label{subsub:exp_parameters}
%The key parameters in our experiments include the number of data parties ($l$), the number of features in each party $i$ ($f_i$), and the categorical value number of each feature ($c_f$). %With a real-life dataset, we will randomly split its features into $l+1$ parties (include $l$ data parties and one task party), so that $\sum f_i$ equals to the total number of features in the dataset. %
%For the number of categorical value in each feature, if the feature is originally a categorical feature, we will keep it as is; if the feature is continuous, we discretize it to four-categories by default according to literature \cite{Brown2012}.
%Note that when we run computation efficiency experiments, we will change $l$, $f_i$, and $c_f$ with simulations to see how they impact the runtime efficiency.


%\begin{figure*}[t]
%\centering
%\begin{minipage}{0.22\textwidth}
%	\includegraphics[width=1\linewidth]{./fig/cmi_fed_agg_correlation.png}
%	\caption{Correlations between Shapley-CMI$_{FED}$ and Shapley-CMI$_{CEN}$}
%	\label{fig:fed_agg_correlation}
%\end{minipage}
%\quad
%\begin{minipage}{.74\textwidth}
%	\begin{subfigure}[t]{.32\linewidth}
%		\includegraphics[width=1\linewidth]{./fig/approx_parkinsons.png}
%		\caption{Parkinsons}
%		\label{fig:approx_parkinsons}
%	\end{subfigure}
%	\begin{subfigure}[t]{.32\linewidth}
%		\includegraphics[width=1\linewidth]{./fig/approx_spect.png}
%		\caption{Spect}
%		\label{fig:approx_spect}
%	\end{subfigure}
%	\begin{subfigure}[t]{.32\linewidth}
%		\includegraphics[width=1\linewidth]{./fig/approx_breast.png}
%		\caption{Breast}
%		\label{fig:approx_breast}
%	\end{subfigure}
%	\vspace{-1em}
%	\caption{Correlation of feature independence (FI) based approximation and original Shapley-CMI. (\textit{Approx\_FI\_full}: approximation with FI assumption on both data and task parties; \textit{Approx\_FI\_data}: approximation with FI assumption on only data parties)}
%	\vspace{-1em}
%	\label{fig:approx}
%\end{minipage}
%\end{figure*}



\subsection{Effectiveness of FedValue}
\label{sub:value_quality}
We evaluate the effectiveness of our FedValue framework from two aspects. We first verify the effectiveness of Shapley-CMI metric in data valuation for a VFL task. We then examine whether the dual-server-aided federated computation mechanism of FedValue can obtain precise Shapley-CMI for each party.
%\subsubsection{Experiment Setup}

\subsubsection{The Effectiveness of Shapley-CMI in Data Valuation}

\textbf{Experimental setup}. Since there is no ground-truth about the data values in real-life practices, we need to carefully design a reasonable reference method to validate the effectiveness of Shapley-CMI. Intuitively, the results of a model-free data valuation method should be comparable to those of the model-dependent ones. However, the valuation results of model-dependent methods often vary with the adopted models~\cite{breiman2001statistical,fisher2019all}. To deal with this, prior research suggests training a set of models and learning an \emph{ensemble feature importance} based on the well-performing ones~\cite{fisher2019all}. Inspired by this, we construct a model-dependent reference method for data party valuation, which takes all the features of a party as an aggregated feature and valuates the party by the \emph{ensemble model-dependent feature importance} of its aggregated feature.

\begin{table}[t!]
	\centering
	\footnotesize
	\caption{Well-performing model selection by prediction accuracy. For each dataset, the accuracy of the best model is in \textbf{bold}; the models with a double-underlined \underline{\underline{accuracy}} would be selected when threshold~$\epsilon=0.02$; all the models with an (both single- and double-) underlined accuracy would be selected when threshold~$\epsilon=0.05$. For example, in the \textit{Parkinsons} dataset, the SVM, GBT, and RF models are selected into $M_{well}$ when $\epsilon$ is set to 0.05.}
	\label{tbl:accuracy}
	\begin{tabular}{@{}llllll@{}}
		\toprule
		& \textit{SVM} & \textit{GBT} & \textit{LR} & \textit{RF} & \textit{NN} \\ \midrule
		\multirow{2}{*}{\textit{Wine}} & \underline{\underline{\textbf{0.967}}} & \underline{0.944} & \underline{\underline{\textbf{0.967}}} & \underline{0.944} & \underline{\underline{\textbf{0.967}}} \\
		& $\pm$0.027 & $\pm$0.030 & $\pm$0.011 & $\pm$0.025 & $\pm$0.041 \\ \midrule
		\multirow{2}{*}{\textit{Parkinsons}} & \underline{0.897} & \underline{\underline{0.908}} & 0.821 & \underline{\underline{\textbf{0.928}}} & 0.856 \\
		& $\pm$0.043 & $\pm$0.053 & $\pm$0.036 & $\pm$0.030 & $\pm$0.058 \\ \midrule
		\multirow{2}{*}{\textit{Spect}} & \underline{\underline{\textbf{0.833}}} & \underline{\underline{0.819}} & \underline{\underline{0.819}} & \underline{\underline{0.822}} & \underline{\underline{0.826}} \\
		& $\pm$0.012 & $\pm$0.032 & $\pm$0.041 & $\pm$0.022 & $\pm$0.045 \\ \midrule
		\multirow{2}{*}{\textit{Breast}} & \underline{\underline{0.951}} & \underline{0.937} & \underline{\underline{\textbf{0.961}}} & \underline{0.937} & \underline{\underline{0.949}} \\
		& $\pm$0.012 & $\pm$0.020 & $\pm$0.007 & $\pm$0.013 & $\pm$0.010 \\ \midrule
		\multirow{2}{*}{\textit{Music}} & \underline{0.605} & \underline{\underline{0.643}} & 0.596 & \underline{\underline{\textbf{0.653}}} & \underline{0.613} \\
		& $\pm$0.021 & $\pm$0.016 & $\pm$0.034 & $\pm$0.024 & $\pm$0.030 \\ \midrule
		\multirow{2}{*}{\textit{Credit}} & \underline{\underline{0.809}} & \underline{\underline{\textbf{0.812}}} & \underline{\underline{0.808}} & \underline{\underline{0.795}} & \underline{\underline{0.805}} \\
		& $\pm$0.004 & $\pm$0.005 & $\pm$0.006 & $\pm$0.006 & $\pm$0.005 \\ \bottomrule
	\end{tabular}
\end{table}

Specifically, we first train a set of prediction models with various machine learning methods, including support vector machine (SVM), gradient boosting decision tree (GBT), logistic regression (LR), random forest (RF), and neural networks (NN). Table~\ref{tbl:accuracy} shows the prediction accuracy of different models on various datasets. Let $acc^*$ denote the best model's accuracy and $\epsilon$ denote a threshold for model selection. For each dataset, we select the models with a prediction accuracy larger than ($acc^*-\epsilon$) as the well-performing ones (denoted as $M_{well}$), where $\epsilon$ is set to $0.02$ and $0.05$ respectively by default. Then, given all well-performing models in $M_{well}$, we use a model-dependent feature importance metric to valuate each party's aggregated feature and average the valuation results by different models as reference. 

In general, Permutation Importance (PI)~\cite{altmann2010permutation} and SHAP~\cite{Lundberg2017} are two widely used model-dependent feature importance metrics. However, it is reported that PI cannot appropriately valuate the data parties that share some features\footnote{A detailed discussion can be found in Sec.~5.6 of \textit{Interpretable Machine Learning} (\url{https://christophm.github.io/interpretable-ml-book/feature-importance.html}).}. In this vein, we ensemble SHAP values of a party's aggregated feature given the well-performing models as a reference of the party's value, denoted as \textit{SHAP-ensemble}. We use the \emph{Pearson correlation} to measure the similarity between Shapley-CMI and SHAP-ensemble, with the assumption that the valuation result of Shapley-CMI should be similar to that of SHAP-ensemble.
%\footnote{It is worth noting that, in a federated learning task, we could not obtain the reference results for practical data valuation, as they require model training on all the parties' data, which violates the common process that data valuation is conducted before model training.}

%\textbf{Comparison settings}.
Based on the evaluation standard, we implement a task party and multiple data parties to carry out experiments on each of the six datasets in Table~\ref{tbl:dataset_stat}. For simplicity, a dataset’s features are randomly and evenly distributed among all the parties in our experiments. Specifically, the number of features in a party is set to 1, 2 and 3, respectively. Besides, we only select 80\% samples of a dataset at random to run an experiment for each setting; by doing so, we can repeat the experiment many (\emph{i.e.}, 50) times with different data samples to obtain the mean and standard deviation of evaluation results for robustness check.

%To compare Shapley-CMI with SHAP-ensemble, we randomly select 80\% samples of a dataset for data valuation in an experiment and repeat this process 5 times. We assume that the parties averagely have 1, 2, or 3 features to facilitate the evaluation, and assign the features of a dataset to different data parties accordingly. If the average feature number is larger than one, we randomly combine the number of features for each party and repeat this feature assignment process for 10 times; otherwise, we assign each data party one feature. We use the open SHAP package\footnote{\url{https://github.com/slundberg/shap}} to calculate SHAP results.

%\color{black}


\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{.9\linewidth}
	\includegraphics[width=1\linewidth]{./fig/correlation5.PNG}
	\caption{Model selection threshold $\epsilon=0.05$}
	\label{fig:ensemble_correlation_1}
	\end{subfigure}
\quad
	\begin{subfigure}[t]{.9\linewidth}
	\includegraphics[width=1\linewidth]{./fig/correlation2.PNG}
	\caption{Model selection threshold $\epsilon=0.02$}
	\label{fig:ensemble_correlation_2}
	\end{subfigure}
	\caption{Correlations between Shapley-CMI and SHAP-ensemble.}
	\label{fig:Shap-Cor}
\end{figure*}

\textbf{Main results}. Fig.~\ref{fig:Shap-Cor} displays the correlations between Shapley-CMI and SHAP-ensemble in data valuation when the well-performing model selection threshold $\epsilon$ is set to 0.05 and 0.02, respectively. We can observe that their data valuation correlations are almost larger than $0.8$ on all datasets under different settings, indicating that Shapley-CMI indeed can effectively valuate each party's contribution in VFL tasks. Recall that the computation of SHAP-ensemble requires data parties to collaboratively train some real models, which could be very costly or even infeasible before the launch of the VFL task. Shapley-CMI avoids specifying any concrete models and thus is more suitable for VFL in practice.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{.95\linewidth}
	\includegraphics[width=1\linewidth]{./fig/correlation_model.PNG}
	\caption{Each party with 1 feature}
	\label{fig:correlation_1}
	\end{subfigure}
	\begin{subfigure}[t]{.95\linewidth}
	\includegraphics[width=1\linewidth]{./fig/correlation_model2.PNG}
	\caption{Each party with 2 features}
	\label{fig:correlation_2}
	\end{subfigure}
	\begin{subfigure}[t]{.95\linewidth}
	\includegraphics[width=1\linewidth]{./fig/correlation_model3.PNG}
	\caption{Each party with 3 features}
	\label{fig:correlation_3}
	\end{subfigure}
	\caption{Correlations between Shapley-CMI and model-dependent SHAP values.}
	\label{fig:correlation}
\end{figure*}

Fig.~\ref{fig:correlation} shows the correlations between Shapley-CMI and SHAP values given various models (denoted as SHAP-$m$ where $m$ can be SVM, GBT, LR, RF, or NN). It is interesting that the correlations between Shapley-CMI and various model-dependent SHAP values are quite different. For example, the correlation of Shapley-CMI with SHAP-GBT is higher than $0.8$ but lower than $0.6$ with SHAP-NN on the Parkinsons dataset. This indicates that the data valuation by SHAP value varies with the adopted models obviously, and some of the model-dependent SHAP values hardly reveal the essential value of a data party. Hence, a model-free data valuation method like Shapley-CMI would be more attractive. Besides, in the experiments we find that Shapley-CMI correlates more with the SHAP values of the high-performance models. For instance, while the model GBT ($0.908$) obtains a higher prediction accuracy than the model NN ($0.856$) does (shown in Table~\ref{tbl:accuracy}), Shapley-CMI has a larger correlation with SHAP-GBT than SHAP-NN on the Parkinsons dataset. This finding further validates the effectiveness of Shapley-CMI for data valuation in VFL.

%Recall the previous example where Shapley-CMI has a larger correlation with SHAP-GBT than SHAP-NN on the Parkinsons dataset. The prediction performance in Table~\ref{tbl:accuracy} shows that model GBT ($0.908$) obtains a higher prediction accuracy than model NN ($0.856$) does. This finding further validates the effectiveness of Shapley-CMI for data valuation in VFL.

%Figure~\ref{fig:aggndcg_by_feature} shows the average \textit{AggNDCG} on all the datasets of our compared methods by varying the feature-number-per-party. In general, our Shapley-CMI consistently performs the best among all the valuation measurements. More specifically, Shapley-CMI's performance improvement is more significant when the feature-number-per-party is smaller (or the party number is largeer). We also observe that, with the increase of the feature-number-per-party (i.e., the decrease of the party number), all the data valuation measurements go up. Note that each valuation measurement is a vector of the size equal to the number of parties; thus, the possible reason of this observation is that diverse measurements may be more easily consistent with each other (higher \textit{AggNDCG}) when the measurement vector size decreases.

%\begin{figure*}[t]
%	\centering
%	\footnotesize
%	\includegraphics[width=.5\linewidth]{./fig/AggNDCG_by_feature_num.PNG}
%	\caption{\textit{AggNDCG} comparison by varying the number of features per party.}
%	\label{fig:aggndcg_by_feature}
%\vspace{-1em}
%\end{figure*}

%Shapley-CMI performs the best and the performance improvement is often statistically significant. In the cases when Shapley-CMI is not the best, there is always no statistical difference between Shapley-CMI and the best measurement. \color{black}  These results indicate that the data valuation measurements of Shapley-CMI are quite correlated to the other model-dependent data valuation measurements. Hence, Shapley-CMI is an effective and representative data valuation method that can be used in federated learning regardless of machine learning models.

\begin{figure*}[t!]
    \centering
	\footnotesize
	\includegraphics[width=.35\linewidth]{fig/cmi_fed_agg_correlation.png}
	\caption{Correlations between Shapley-CMI$_{FED}$ and Shapley-CMI$_{CEN}$.}
	\label{fig:fed_agg_correlation}
\end{figure*}

\subsubsection{The Effectiveness of Dual-server-aided Federated Computation}
Ideally, FedValue's Shapley-CMI computation with the designed dual-server-aided federated computation mechanism (denoted as Shapley-CMI$_{FED}$) should %theoretically 
obtain the same results as the centralized Sharpley-CMI computation when all parties' data can be gathered (denoted as Shapley-CMI$_{CEN}$). We here empirically compare Shapley-CMI$_{FED}$ with Shapley-CMI$_{CEN}$ by Pearson correlation. 

Fig.~\ref{fig:fed_agg_correlation} shows the correlations of data valuation results between Shapley-CMI$_{FED}$ and Shapley-CMI$_{CEN}$ on all datasets. The observation verifies that Shapley-CMI$_{FED}$, which allows all parties to preserve their own raw data, can achieve exactly the same data valuation results as Shapley-CMI$_{CEN}$, which needs to aggregate all parties' data. These results validate the effectiveness of the designed dual-server-aided federated computation paradigm in FedValue.

%\subsection{Approximation Performance}
%In this section, we test how the approximation techniques proposed in Sec.~\ref{sub:approximate_CMI} will impact the valuation quality. How the approximation methods accelerate the computation efficiency will be illustrated in the next Sec.~\ref{sub:exp_efficiency}.
%We use three datasets as the representatives to evaluate the approximations, i.e., \textit{Spect}, \textit{Parkinsons}, and \textit{Breast}.

%\subsubsection{Feature independence-based approximation} We have implemented two variants of the feature independence-based approximation, namely \textit{Approx-FI-full} (feature independent assumption in task and data parties, Eq.~\ref{eq:approx_2}) and \textit{Approx-FI-data} (feature independent assumption only in data parties, Eq.~\ref{eq:approx_1}). We calculate the correlation between the approximated and the original Shapley-CMI to indicate their similarity. We repeat the computation for 10 times and record the average correlation. We randomly split the features into $l+1$ groups if there are $l$ data parties and one task party. %The results are shown in Fig.~\ref{fig:approx}.



%Then, we compute Shapley-CMI and the approximations, \textit{Approx-FI-full} and \textit{Approx-FI-data}, for all the data parties. Finally, we calculate the correlations between all the parties' Shapley-CMI and \textit{Approx-FI-full}/\textit{Approx-FI-data}. This process is repeated for 10 times and the average correlation is recorded.

%Fig.~\ref{fig:approx} shows the results that, with the increase of the data party number, the correlations of the approximation and Shapley-CMI also increase. The reasons might be, with the increase of data parties, each party's feature number is reduced, so that the feature independence assumptions can be (partially) met with a higher probability. Besides, by comparing \textit{Approx-FI-full} to \textit{Approx-FI-data}, we find that \textit{Approx-FI-data} is much more correlated to the original Shapley-CMI, as it does not make the feature independence assumption on the task party features. Particularly, for all the three datasets, \textit{Approx-FI-data} can achieve more than $0.9$ correlation with the original Shapley-CMI for 5 data parties. Hence, if the computation overhead is acceptable (e.g., the task party feature number is not large), we suggest making FI assumptions only on data parties to generate a better approximation effect.




%\vspace{-1em}

%\subsubsection{Feature dimension reduction} We use PCA to reduce data parties' feature dimension to the half of the original dimension, and conduct the experiments with 3 data parties. The results are shown in Fig.~\ref{fig:approx_pca}. Interestingly, the results on the three datasets show distinct patterns. In Parkinsons, applying PCA to reduce feature dimensions decreases the correlations with the original Shapley-CMI; in Spect, leveraging PCA significantly increases the correlations; in Breast, the impacts of PCA are slight and opposite for \textit{Approx\_FI\_full} and \textit{Approx\_FI\_data}. This tells that in practice, how the feature reduction technique (e.g., PCA) impacts the data valuation quality is non-trivial, and deeper investigations are needed in the future.
%\vspace{-1em}


\subsection{Computational Efficiency of FedValue}
\label{sub:exp_efficiency}
%While FedValue is composed of the Shapley-CMI metric and its dual-server-aided federated computation mechanism, w
There are two classes of key parameters that may influence the computational efficiency of FedValue. The first class of parameters relates to the Shapley-CMI computation, including the numbers of data parties, features and data samples. The other class of parameters is set against the malicious servers, including the ID duplication times and the randomized adversarial data samples. We vary the parameters to examine the computation efficiency of FedValue. By default, there are 5 data parties; every data party holds a binary feature, while the task party owns a binary feature and a binary task label; the total number of samples is 100,000, including 10\% (10,000) real data samples and 90\% (90,000) adversarial data samples; the ID duplication times is set to 3. The experimental platform is an ordinary laptop with AMD Ryzen R7 4800HS (2.9GHz) and 16GB RAM.

\begin{figure*}[t!]
	\centering
    \begin{subfigure}[t]{.3\linewidth}
		\includegraphics[width=1\linewidth]{./fig/runtime-parties.png}
		\caption{data parties}
		\label{fig:runtime_multi_parties}
	\end{subfigure}
\quad
	\begin{subfigure}[t]{.3\linewidth}
		\includegraphics[width=1\linewidth]{./fig/runtime-feature-categories.png}
		\caption{A data party's features}
		\label{fig:runtime_two_parties_feature_cat}
	\end{subfigure}
\quad
	\begin{subfigure}[t]{.3\linewidth}
		\includegraphics[width=1\linewidth]{./fig/runtime-data-sample.png}
		\caption{Real data samples}
		\label{fig:runtime_data_sample}
	\end{subfigure}
	\caption{Computation time with varied Shapley-CMI related parameters.}
	\label{fig:runtime_Shapley}
\end{figure*}


\begin{figure*}[t!]
	\centering
    \begin{subfigure}[t]{.3\linewidth}
		\includegraphics[width=1\linewidth]{./fig/runtime-copy-times.png}
		\caption{ID duplication times}
		\label{fig:runtime_copy_times}
	\end{subfigure}
\quad\quad
	\begin{subfigure}[t]{.3\linewidth}
		\includegraphics[width=1\linewidth]{./fig/runtime-adversarial-data-sample.png}
		\caption{Adversarial data samples}
		\label{fig:runtime_adversary_data}
	\end{subfigure}
	\caption{Computation time with varied privacy-preserving related parameters.}
	\label{fig:runtime_Privacy}
\end{figure*}

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=.4\linewidth]{./fig/runtime-parties.png}
%	\caption{Computation time of multiple data parties. Shapley sampling uses 10,000 samplings. }
%	\label{fig:runtime_multi_parties}
%\end{figure*}
Fig.~\ref{fig:runtime_Shapley} shows the computation time of FedValue with three varied parameters for Shapley-CMI computation. In particular, Fig.~\ref{fig:runtime_multi_parties} and Fig.~\ref{fig:runtime_two_parties_feature_cat} report the computation time over the number of data parties and the number of a party's features, respectively. %Note that the computation time is calculated by (i) recording the time of simulating the multi-server computation for one permutation of data parties and (ii) multiplying the time with the number of permutations\footnote{$n!$ for original Shapley-CMI and 5,000 for Shapley sampling.}.  %Note that we use the log scale for the computation time.
The results show that the computation time of FedValue increases almost exponentially with the two parameters.
%This is mainly because the Shapley-CMI computation needs to enumerate all the permutations of parties. 
These observations suggest the importance of using practical techniques to reduce the computation time when there are a large number of data parties or the parties possess many features. %For example, when the number of data parties is 12, the original Shapley-CMI computation needs more than $10^{10}$ seconds; with Shapley sampling, the computation time is shorter than $10^6$ seconds.
%Besides, Fig.~\ref{fig:runtime_two_parties_feature_cat} shows that the computation time of Shapley-CMI goes up exponentially by the feature number of the data party increases.
Fig.~\ref{fig:runtime_data_sample} shows that the running time of FedValue increases linearly with the number of data samples. Specifically, for a VFL task with 100,000 data samples (10,000 real samples and 90,000 adversarial samples) and 5 parties, we can obtain the valuation results in 10 minutes; even if the number of data samples increases to 1,000,000 (100,000 real samples and 900,000 adversarial samples), the computation time is not beyond 2 hours.% In other words, the number of data samples is not a parameter that diminishes the efficiency of FedValue significantly.
%With our proposed feature independence-assumed approximation method (FI-approx-all and FI-approx-data), the computation complexity is then linear to the number of features, which can significantly reduce the computation time when the number of features becomes large. \color{blue}It is also worth noting that, if the feature number of one party is small, using FI approximation may not accelerate the computation. The reason is that FI approximation leverages \textit{many simple} mutual information calculations to replace \textit{one complicated} mutual information calculation; if the complicated mutual information computation is not time-consuming (i.e., the feature number is small), FI approximation may not reduce computation time.

% by varying different parameters including the number of features, data samples, and ID duplication times.

Fig.~\ref{fig:runtime_copy_times} and Fig.~\ref{fig:runtime_adversary_data} show how the computation time of FedValue varies with the ID duplication times and the number of adversarial data samples, respectively. These two parameters essentially control the overall amount of data used in the computation. It is common sense that adding more data would sacrifice the computation efficiency for the protection of data privacy. Nevertheless, we observe that the computation time is also linearly associated with both of the privacy-preserving parameters. %We note that these two parameters essentially control the overall amount of data used in the computation. %Therefore, the results further verify that the computation time varies linearly over the amount of data used in data valuation.

%With the increasing number of data samples (Fig.~\ref{fig:runtime_two_parties_data_sample}) and ID duplication times (Fig.~\ref{fig:runtime_two_parties_copy_time}), the running time of our method increases linearly. It is worth noting that, for over one million data samples, we can still obtain the valuation measure in one minute. Meanwhile, when the feature number of the data party increases (Fig.~\ref{fig:runtime_two_parties_feature_cat}), the computation time of Shapley-CMI goes up exponentially. With our proposed feature independence-assumed approximation method (FI-approx-all and FI-approx-data), the computation complexity is then linear to the number of features, which can significantly reduce the computation time when the number of features becomes large. \color{blue}It is also worth noting that, if the feature number of one party is small, using FI approximation may not accelerate the computation. The reason is that FI approximation leverages \textit{many simple} mutual information calculations to replace \textit{one complicated} mutual information calculation; if the complicated mutual information computation is not time-consuming (i.e., the feature number is small), FI approximation may not reduce computation time.\color{black}

%\color{blue}  In particular, the computation time on our experiment platform is roughly $0.17\cdot 2^k second$ where $k$ is the feature number. Then, a data party with $20$ features will need around $50$ hours for Shapley-CMI computation, which is impractical. Hence, if a data party has a large number of features, we suggest conducting feature dimension reduction first. We also believe that other acceleration techniques (e.g., feature independence assumptions \cite{Brown2012}) deserve more investigations in the future.



%\color{black}
%This also illustrates the necessity of applying approximations, such as Shapley sampling (Sec.~\ref{subsub:shapley_sampling}), to boost the computation in practice.

%In the next subsection, we will test our approximation techniques.

\subsection{The Effectiveness of Practical Computation Techniques}
Here, we evaluate the practical computation techniques for FedValue acceleration. 
%We have observed in the prior experiments that the computation overhead of FedValue is nearly exponential to the number of data parties as well as the number of a party's features. While we have proposed some practical computation techniques to facilitate the federated Shapley-CMI computation, we evaluate these techniques' effects in this section. 
In particular, we compare the data valuation results in terms of Shapley-CMI between the original FedValue and the FedValue that adopts any practical computation techniques (denoted as fast-FedValue). On one hand, we expect that the data valuation results of fast-FedValue could be close to those of the original FedValue. Accordingly, we adopt the MAPE (Mean Absolute Percentage Error) measure to characterize this closeness. On the other, we expect that the computation efficiency of FedValue could be improved with practical computation techniques. Since the datasets \emph{Breast} and \emph{Music} in Table~\ref{tbl:dataset_stat} have the largest numbers of features, we use them as the representatives to examine the techniques of Shapely sampling and feature dimension reduction.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{.37\linewidth}
		\includegraphics[width=1\linewidth]{./fig/approx_sampling.png}
		\caption{MAPE}
		\label{fig:sampling_mape}
	\end{subfigure}
	\quad	\quad
	\begin{subfigure}[t]{.37\linewidth}
		\includegraphics[width=1\linewidth]{./fig/sampling_time.png}
		\caption{Computational Overhead}
		\label{fig:sampling_time}
	\end{subfigure}
	\caption{Performance of FedValue using Shapley sampling.}
	\label{fig:sampling}
\end{figure*}


\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{.37\linewidth}
		\includegraphics[width=1\linewidth]{./fig/pca_error_by_component.PNG}
		\caption{MAPE}
		\label{fig:approx_pca_error}
	\end{subfigure}
	\quad	\quad
	\begin{subfigure}[t]{.37\linewidth}
		\includegraphics[width=1\linewidth]{./fig/pca_time_by_component.PNG}
		\caption{Computational Overhead}
		\label{fig:approx_pca_time}
	\end{subfigure}
	\caption{Performance of FedValue using PCA (\#data parties = 5).}
	\label{fig:approx_pca}
\end{figure*}

%Interestingly, the results on the three datasets show distinct patterns. In Parkinsons, applying PCA to reduce feature dimensions decreases the correlations with the original Shapley-CMI; in Spect, leveraging PCA significantly increases the correlations; in Breast, the impacts of PCA are slight and opposite for \textit{Approx\_FI\_full} and \textit{Approx\_FI\_data}. This tells that in practice, how the feature reduction technique (e.g., PCA) impacts the data valuation quality is non-trivial, and deeper investigations are needed in the future.


\textbf{Shapley sampling}. %Actually, the results in Sec.~\ref{sub:value_quality} have already applied Shapley sampling (10,000 samplings) to accelerate computation.
Theoretically, the fast-FedValue with Shapley sampling cannot attain precise Shapley-CMI if the number of Shapley sampling is small. The increase of samplings will decrease the Shapley-CMI differences (MAPE) between the fast-FedValue and the original FedValue. Therefore, we have interests in how many samplings can help fast-FedValue achieve a small enough MAPE value. 
%We use Parkinsons, Spect, and Breast datasets, and follow the setting in Sec.~\ref{sub:value_quality} to calculate sampled Shapley-CMI. %Fig.~\ref{fig:sampling} shows how sampled Shapley-CMI changes with the increase of samplings. As Shapley-CMI is a vector of parties' valuations and hard to visualize, we compute the entropy of Shapley-CMI to show how sampled Shapley-CMI changes with the size of samplings in Fig.~\ref{fig:sampling}.
Fig.~\ref{fig:sampling_mape} displays how the MAPE of Shapley-CMI between FedValue and fast-FedValue changes with the number of samplings. The results show that the MAPE drops dramatically when the number of samplings increases from 100 to 1200, and it steadily converges towards a small value if the number of samplings continues growing. Fig.~\ref{fig:sampling_time} reports how the number of samplings would affect the efficiency of Shapley-CMI computation. We notice that the computation time is nearly linear to the number of samplings. By integrating both observations regarding effectiveness and efficiency evaluations, we leverage 5,000 samplings for Shapley-CMI computation in our experiment, as it can achieve a small MAPE within tolerable computation time.

\textbf{Feature dimension reduction}. %We randomly split the dataset features into $|\bm {\mathcal D}|+1$ groups, where $|\bm {\mathcal D}|$ is the number of data parties and 1 indicates the task party ($|\bm {\mathcal D}|=5$ in this experiment). 
In this experiment, we construct fast-FedValue using PCA to reduce the feature dimensions of data parties. Fig.~\ref{fig:approx_pca_error} displays that the MAPE between FedValue and fast-FedValue decreases rapidly when the retained number of PCA components increases from 2 to 4. This observation indicates that the fast-FedValue can better approximate the true Shapley-CMI when it keeps more informative components. Fig.~\ref{fig:approx_pca_time} compares fast-FedValue and FedValue by the computation time. We can observe that the computation time of FedValue can be decreased exponentially when each party holds less number of PCA components. In brief, there exists a trade-off between the effectiveness and efficiency of FedValue by leveraging feature dimension reduction techniques.

%We use PCA to reduce data parties' feature dimension, and compare the PCA Shapley-CMI to the original one by calculating MAPE (Mean Absolute Percentage Error).  We repeat the computation for 10 times and record the average MAPE; in particular, we randomly split the dataset features into $|\bm {\mathcal D}|+1$ groups supposing $|\bm {\mathcal D}|$ data parties and one task party ($|\bm {\mathcal D}|=5$ in this experiment). The results are shown in Fig.~\ref{fig:approx_pca_error}. We observe that the MAPE ranges from 5\% to 13\% under different number of PCA components retained. Specifically, with the increase of PCA components, the MAPE will be smaller, as PCA can approximate the original features better. We also record the computation time ratio of PCA Shapley-CMI and the original one, as shown in Fig.~\ref{fig:approx_pca_time}. The computation time ratio is always smaller than 1, as the size of PCA-decomposed features is smaller than the size of original features. Moreover, with the increase of PCA components, each party holds more PCA-decomposed features, and thus the computation time also increases.

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=.45\linewidth]{./fig/fi_approx_pca.PNG}
%	\caption{Feature independence-assumed Shapley-CMI approximation on PCA features (\#data parties = 5, \#PCA components = 3). }
%	\label{fig:fi_approx_pca}
%\end{figure*}

%\textbf{Feature independence-assumed approximation}. We have implemented two variants of the feature independence-assumed approximation, namely \textit{FI-Approx-all} (feature independent assumption in task and data parties, Eq.~\ref{eq:approx_2}) and \textit{FI-Approx-data} (feature independent assumption only in data parties, Eq.~\ref{eq:approx_1}). We calculate MAPE between the approximated and the original Shapley-CMI to indicate their similarity. As PCA can decompose each party's features into (roughly) independent ones and this fits the feature independence assumption better, this experiment is conducted for PCA features. The results are shown in Fig.~\ref{fig:fi_approx_pca}. Interestingly, the results on the two datasets show distinct patterns. In Breast, applying FI approximation on PCA features increases MAPE from the original Shapley-CMI; in Music, the result is the opposite. The possible reason is that diverse correlations exist between various parties' features for different datasets. Hence, in practice, how FI approximation techniques impact Shapley-CMI computation is non-trivial, and deeper investigations are needed in the future. Besides, using FI approximation may accelerate computation when the feature number of one party is large; we will elaborate on this in the next subsection.



%\color{black}



==> VFLValue AIJ/intro.tex <==
\section{Introduction}
%With the emergence of various data regularization laws all around the world (e.g., General Data Protection Regulation\footnote{\url{https://gdpr.eu/eu-gdpr-personal-data}}), privacy has become one of the most fundamental issues in building big data applications. Especially, if different parts of data are stored in diverse parties, then the raw data cannot be directly exchanged with each other under the up-to-date data regulations. This brings novel challenges for the big data and machine learning community, as fusing heterogeneous data from multiple parties is prerequisite for building powerful data-driven applications.

%Recently, the federated learning (FL) \cite{konevcny2016federated,yang2019federated} paradigm is proposed to enable distributed collaborative learning on multiple parties' data without leaking any party's raw private data. Basically, FL lets each party do local computation on their private data, and then transfer only non-sensitive information (e.g., gradients) to other parties for collaborative machine learning. There are two main types of FL, i.e., vertical FL (VFL) and horizontal FL (HFL). In VFL, different parties have different features for the same set of data samples. For example, a bank can collaborate with a mobile network operator by VFL, where the mobile network operator can provide users' features like phone bills and frequently-visited locations to help the bank conduct credit assessment \cite{han2019creditprint}. In HFL, parties share the same feature space but differ in sample space;to train a local model, and a federated model is eventually learned with parameters in all the parties. For instance, Google GBoard uses HFL to train a federated keyboard query prediction model \cite{yang2018applied}.

%{\color{blue} %While there is an increasing interest in collaborative machine learning with fused data from multiple parties, data privacy and security have drawn world-wide attention. Specially, various data regularization and laws (e.g., General Data Protection Regulation\footnote{\url{https://gdpr.eu/eu-gdpr-personal-data}}) have been recently enacted to enforce data privacy and forbid raw data's fusing. \textit{Federated learning} (FL) is an emerging paradigm towards privacy-preserving collaborative machine learning~\cite{konevcny2016federated,yang2019federated}. Basically, FL lets various parties perform local computations with their private data and only communicate insensitive information (e.g., gradients) with others. It takes benefits from all parties' data to achieves comparative machine learning performance without leaking any party's data assets.

Recent years have witnessed an increasing interest in collaborative machine learning with data fused from multiple data holders for Artificial Intelligence (AI) applications~\cite{FATE_JMLR,FISCH201290}. In practice, however, it is yet very hard to integrate data from different parties, owing to industry competitions, security requirements or sophisticated administrative procedures~\cite{FATE_JMLR,yang2019federated}. %For one thing, data privacy and security have drawn world-wide attention. Various data regularization and laws (e.g., General Data Protection Regulation\footnote{\url{https://gdpr.eu/eu-gdpr-personal-data}}) have been recently enacted to enforce data privacy and forbid raw data's fusing. Besides, data are becoming one of the most valuable capitals, data holders are often reluctant to transporting their own data assets to others and losing controls on the data.
\emph{Federated learning} (FL) is an emerging paradigm towards privacy-preserving collaborative machine learning~\cite{yang2019federated,konevcny2016federated}. Basically, FL allows various parties to perform local computations on their private data and only communicate insensitive information, \emph{e.g.}, gradients of self-learned deep neural networks~\cite{mcmahan2017communication}, with others. It benefits from all parties' data to achieve high-performance machine learning without leaking any party's data assets.

Horizontal FL (HFL) and vertical FL (VFL) are two typical types of FL mechanisms~\cite{yang2019federated}. %regarding FL parties' shared data spaces.
In HFL tasks, various parties share a same set of features and perform secure collaborative learning with different data samples~\cite{Wei2020,Song2019,Wang2020}. %For instance,In HFL, all the parties can independently train a local model and improve their model by sharing the parameters securely~\cite{yang2018applied}.
Comparatively, parties in VFL tasks own different features for a same set of data samples, and collaboratively learn models by taking advantage of integrated features from other parties~\cite{wu2020,Wang2019}. While existing FL studies focus more on HFL to alleviate the training data scarcity problem, VFL is also requisite to many practical data-driven businesses~\cite{wu2020}. For example, banks may willingly collaborate with mobile network operators or online commerce platforms, to collect more indicative information (\emph{e.g.}, phone bills and shopping logs) about their customers and improve credit assessment performance~\cite{han2019creditprint}. In brief, if any party (namely \emph{task party}) needs to train a better business model via exploiting more feature information about its data samples, it can launch a VFL task by inviting some parties with valuable data (namely \emph{data parties}).% Besides, the design of VFL may be also more challenging as some of parties in VFL may only have features but not be able to train local models.

This work concentrates on VFL tasks, which are widely needed in practice but still under-investigated~\cite{wu2020}. In particular, %different from the stream of research in designing privacy-preserving decentralized collaborative learning schemes~\cite{hardy2017private,wu2020}, 
it attempts to tackle a fundamental issue in VFL: \textit{data valuation}, which aims at quantifying the potential contributions of different data parties to a specific VFL task, given the task party's self-owned data and before the launch of the VFL task. %In other words, it learns how much a task would get improved if a task party collaborates with other data parties. 
On one hand, data valuation can help task parties to determine which data parties are valuable to collaborate with for a specific task. On the other, it can help to incentivize high-quality data parties to join a VFL task if their contributions can be fairly priced, which is deemed crucial to the success of building legal data marts~\cite{yang2019federated}. %we note that data parties in a VFL task barely partake in any model improvement from collaboration; thus, how to incentivize data parties fairly with respect to their contributions in the task is an essential issue to the success of a VFL task. 
In this vein, data valuation can provide the imperative information for establishing contribution-based incentive mechanisms, so that both the task party and data parties in a VFL task can gain fair benefits. %Generally speaking, data valuation is important for data pricing, collaboration decision-making, firm valuation

The problem of data valuation in VFL, however, is non-trivial and presents two unique challenges. The first challenge comes from building a task-specific but model-free data valuation method. Some context-independent metrics have been proposed to valuate data by their intrinsic properties, including completeness, precision, uniqueness or timeliness~\cite{batini2009methodologies}, which however cannot estimate how much each of the data parties can improve a specific business task and therefore can hardly be used for precise data pricing. In this sense, a \emph{task-specific} data valuation metric that can help differentiate the contribution of various parties is in great need for a VFL task. There also exist some context-aware feature importance methods, \emph{e.g.}, SHAP value~\cite{Lundberg2017}, that can be applied to valuate data parties; but they often depend on running a bundle of specific models, which is typically infeasible in the early stage of an FL collaboration where basic trusts between different parties are still missing. % However, data valuation is often required for party selections and determinations in the early stage of a potential FL collaboration before model training. %arbitrary models like logistic regression~\cite{hardy2017private} or boosting tress~\cite{Cheng2019SecureBoostAL,wu2020} could be applied for a VFL task, which is often hardly determined in the early data valuation phase for possible collaboration.
Therefore, a \emph{task-specific} but \emph{model-free} data valuation measure is urgently required for VFL.

The second challenge comes from the privacy-preserving requirement for data valuation in VFL. In principle, data valuation for a VFL task should be mandatorily compliant with data protection regulations and should prevent the leakage of raw data from any parties. However, assessing the contributions of data parties in collaborative modeling often requires some knowledge about parties' interactions, such as data correlations. How to acquire the interactive information among various parties without disclosing their raw data remains a great challenge. The secure multiparty computation (MPC) protocols provide a promising solution by introducing some third-parties for privacy-preserving data valuation, but some key points remain unaddressed. For example, what information can or must be transmitted to achieve data valuation without privacy leakage, and what if the third-parties are not completely trustworthy, \emph{e.g.}, honest-but-curious or even malicious. Hence, to protect data valuation from being violated by third-party servers' malicious behaviors in an MPC framework also needs a delicate design.
%}

This paper overcomes the above challenges and makes several contributions:

$\bullet$ To the best of our knowledge, this is the first work that proposes a  privacy-preserving, task-specific and model-free data valuation mechanism, named FedValue, for VFL tasks.

$\bullet$ We propose a novel data valuation metric Shapley-CMI for FedValue based on both information theory and game theory. Shapley-CMI can effectively quantify multiple data parties' values in a specific learning task without relying on any particular model.

$\bullet$ We also design a novel dual-server-aided federated computation mechanism for FedValue, which can accomplish federated computation of Shapley-CMI without leaking any party's raw data. Besides, we also demonstrate how to use some computational acceleration methods to enhance the efficiency and scalability of FedValue.

We conduct extensive experiments on six real-life datasets and verify the effectiveness of FedValue for data valuation in VFL. The results demonstrate that Shapley-CMI can effectively valuate data parties given a specific task, and the dual-server-aided federated computation mechanism can precisely compute Shapley-CMI in a privacy-preserving manner. Moreover, we evaluate the computational efficiency of FedValue by various parameters, such as the numbers of data samples, features in a party as well as data parties, and show the effects of acceleration techniques for practical FedValue computation. In particular, we show that FedValue can compute Shapley-CMI for a VFL task with five parties and 100,000 samples in 10 minutes by a laptop with ordinary configurations.

%We conduct extensive experiments on six real-life datasets. Results validate that our proposed Shapley-CMI outperforms model-specific feature valuation metrics, such as SHAP \cite{Lundberg2017} and Permutation Importance \cite{altmann2010permutation}, by achieving better generalizable valuation quality. The scalability test shows that for five data parties and 100,000 samples, FedValue can efficiently compute Shapley-CMI in only 10 minutes with the computing power of an ordinary laptop.


==> VFLValue AIJ/method.tex <==


%even with the distributed NMI-based metric computation process, we prove that certain private data can be disclosed during the computation process (Sec. XXX). To this end, we have adopted the homomorphic encryption techniques to ensure the computation intermediate results secret. Particularly, we adopt the threshold variant of the homomorphic encryption so that the encrypted data can only be decrypted with the agreement of all the parties, so that our mechanism can fight against party collusion attacks.

% The key novelty of our proposed data quality metric is its independence of specific models

\section{Method: FedValue}

%In this section, we elaborate on the design of FedValue. We will first introduce the computation process of CMI-based data value metric assuming that all the parties' data can be collected together with the Shapley value idea in the game theory \cite{shapley1953value}, denoted as \textit{Shapley-CMI}. Then, we illustrate how to compute Shapley-CMI in a privacy-preserving distributed manner. Finally, we describe how to approximate Shapley-CMI in practice when the number of features and parties is large.


%In this section, we overview the design of our proposed data valuation method for VFL, named \textit{FedValue}.

%\subsection{Method Overview}
In this section, we propose \emph{FedValue}, a privacy-preserving, task-specific but model-free framework, for fair data valuation in a VFL task. Two major components of FedValue, \emph{i.e.}, a data valuation metric and a federated computation mechanism for the metric, are carefully designed with this purpose. Concretely, given a specific learning task, we first design a model-free metric to assess the value of data provided by various data parties without considering the data privacy issue. We then discuss how to compute the metric in a VFL system where the raw data of any party must be preserved locally for privacy concerns. Finally, some techniques are proposed to accelerate FedValue in practice.

%First, to achieve model-free data valuation, we propose a CMI (conditional mutual information) \cite{Brown2012}  based feature valuation method. In particular, we design a Shapley-CMI metric which can quantify data contribution for multiple parties, inspired by the Shapley values originated from the game theory \cite{shapley1953value}.  % Compared to existing data quality metrics such as Shapley value, our NMI-based value has two distinct advantage of not dependent on the specific training models. %Moreover, our NMI-based value can ensure some nice properties that

%Second, for computing the Shapley-CMI metric without transferring the raw data between parties, we propose a distributed Shapley-CMI computation process. In particular, the most difficult part in computing Shapley-CMI in VFL is its necessity to calculate a joint (conditional) probability of multiple variables in different parties. To address this challenge, we design a dual-server-aided PSI (Private Set Intersection \cite{Kamara2014ScalingPS}) method for entropy computation of a joint probability. %Moreover, since the entropy of continuous features is hard to compute, we propose a xxx based discretization method to convert a continuous feature to a discrete one.

%\textbf{Finally, approximation ...}

\subsection{Data Valuation Metric}
As stated in Section~\ref{sec:problem}, it is non-trivial to value a data party for a VFL task in a task-specific but model-free manner. The valuation task becomes even more challenging when we consider the involvement of multiple data parties. We therefore begin with the data valuation of only one data party, and then design a general metric that can take account of multiple data parties.

\subsubsection{Metric with One Data Party} 
%Intuitively, we can take the \emph{marginal improvement} of a feature to the overall modelling performance as the data value of the feature. Along this line, for any data party $d$ with features $\bm{X}_d$, the data value of $\bm{X}_d$ can be formulated as
%\begin{equation}
%    V(\bm{X}_d)=val(\bm{X}_d\cup\bm{X}_t,y_t)-val(\bm{X}_t,y_t)
%\end{equation}
Suppose we have a task party $t$ who owns features $\bm{X}_t$ and task label $Y_t$, and a data party $d$ who owns features $\bm{X}_d$. Intuitively, we can take the \emph{marginal improvement} of $\bm{X}_d$ to the overall \emph{modelling performance} as the data value of $\bm{X}_d$. This idea, however, requires to specify the learning model and therefore violates the model-free constraint. 

An alternative method is to approximate the modelling performance with the \emph{coupling tightness} between $\bm{X}_d$ and the task label $Y_t$, denoted as $C(\bm{X}_d,Y_t)$, which not only avoids running specific models but also meets the task-specific requirement by using $Y_t$. Nevertheless, $C(\bm{X}_d,Y_t)$ might still over-estimate the contribution of $\bm{X}_d$ for it might correlate positively with the task party's self-owned features $\bm{X}_t$. Therefore, we should pursue a more accurate metric formulated like $C(\bm{X}_d,Y_t;\bm{X}_t)$, which is the coupling tightness of $\bm{X}_d$ with respect to $Y_t$ given the already possessed $\bm{X}_t$. Note that when there is only one data party $d$, the marginal improvement of $\bm{X}_d$ to the modelling performance is right $C(\bm{X}_d,Y_t;\bm{X}_t)$, and the remainder of our work is to define a proper $C$ function.

Conditional Mutual Information (CMI), a fundamental metric used for feature selection~\cite{Brown2012}, is an excellent candidate of the $C$ function. Basically, CMI measures the shared information between two variables given a third variable. In the VFL case with only one data party, CMI can be properly applied to assess the coupling tightness between the task label $Y_t$ and the data party's features $\bm {X}_d$ given the task party's features $\bm X_t$, and written as:
\begin{equation}
	I(\bm {X}_d;Y_t| \bm X_t)  = \sum_{\bm x_t \in \bm {\mathcal X}_t} p(\bm x_t) \sum_{\bm {x}_d \in \bm {\mathcal X}_d} \sum_{y_t \in \mathcal Y_t} p(\bm {x}_d y_t| \bm x_t) \log \frac{p(\bm {x}_d y_t|\bm x_t)}{p(\bm {x}_d|\bm x_t)p(y_t|\bm x_t)},
	\label{eq:cmi}
\end{equation}
where $\bm {\mathcal X}_d$, $\bm {\mathcal X}_t$, and $\mathcal Y_t$ denote the sets of possible values of $\bm {X}_d$, $\bm {X}_t$, and $Y_t$, respectively.

According to Eq.~\eqref{eq:cmi}, we need to estimate the distributions of $p(\bm {x}_d y_t| \bm x_t)$, $p(\bm {x}_d|\bm x_t)$ and $p(y_t|\bm x_t)$ for CMI computation. For discrete features, the \emph{maximum likelihood} method, which divides the occurrence frequency of $\bm x_t$ by the total number of data samples, can be adopted to estimate these distributions. As for continuous features, we can convert them to discrete ones and then apply the maximum likelihood method for estimation. %\footnote{Directly estimating the distribution of continuous features (i.e., not being discretized) needs to assume the underlying models (e.g., Gaussian mixture models) \cite{Brown2012}. Since it is non-trivial to find appropriate model assumptions for practical applications, we leave the estimation of (non-discretized) continuous feature distributions to the future work.}.  %\textit{Maximum likelihood}, dividing the occurrence frequency of $\bm x$ by the total number of data samples, is a widely-used way to estimate the distribution for discrete data $p(\bm X = \bm x)$. With this maximum likelihood probability estimation,
In this vein, the CMI can be computed as:
\begin{equation}
	\hat I(\bm {X}_d;Y_t| \bm X_t) = \sum_{\bm {x}_d \in \bm{\mathcal X}_d} \sum_{\bm {x}_t\in  \bm{\mathcal X_t} } \sum_{y_t \in \mathcal Y_t} \hat{p}(\bm {x}_d\bm {x}_t y_t) \log \frac{\hat p(\bm {x}_d y_t|\bm x_t)}{\hat p(\bm {x}_d|\bm x_t)\hat p(y_t|\bm {x}_t)}
	\label{eq:cmi_ml1}
\end{equation}
\begin{equation}
	= \frac{1}{n} \sum_{\bm {x}_d \in \bm{\mathcal X}_d} \sum_{\bm {x}_t\in  \bm{\mathcal X_t} } \sum_{y_t \in \mathcal Y_t} N(\bm {x}_d\bm {x}_t y_t) \log \frac{N(\bm{x}_t) N(\bm{x}_d y_t \bm{x}_t)}{N(\bm{x}_d \bm{x}_t) N(y_t\bm{x}_t)},
	\label{eq:cmi_ml2}
\end{equation}
where $\hat p$ is the maximum likelihood probability estimation, $ N(\cdot)$ is the number of data samples with the given variable values, and $n$ is the total number of data samples. Note that CMI can be estimated by Eq.~\eqref{eq:cmi_ml2} precisely when the number of data samples gets sufficiently large, referring to the Strong Law of Large Numbers~\cite{Brown2012}. %However, when the feature dimension of $\bm {X}_d$ or $\bm {X}_t$ increases, the reliability of the estimated probability decreases. We will discuss some alternative methods to deal with the high-dimensional data in practice later in Sec.~\ref{sub:approximate_CMI}.

\emph{Remark}.~The CMI in Eq.~\eqref{eq:cmi_ml1} is a task-specific but model-free metric. Compared with model-dependent metrics like SHAP value~\cite{Lundberg2017}, the computation of CMI in Eq.~\eqref{eq:cmi_ml2} could be much more efficient without running models physically, and the loss of valuation precision is tolerable, as will be shown in our experimental part. It is also noteworthy that the computation of CMI is non-trivial in the VFL setting as $\bm{X}_d$ and $\bm X_t$ ($Y_t$) are typically stored in two parties privately. We will revisit this point in Section~\ref{sub:fed_computation_cmi}.

\subsubsection{Metric for Multiple Data Parties}
Although CMI can be used for data valuation when there is only one data party; it cannot be directly applied to the VFL scenarios with multiple data parties. One may suggest separately valuating each of the multiple data parties in a VFL task and taking the sum of a set of data parties' values as their aggregated value to the task party. Nevertheless, this method neglects the feature correlations among data parties and likely leads to inaccurate data valuation for the parties' collaborative modeling. To consider the correlations, one may assume data parties enter the VFL system orderly and then sequentially valuate a data party conditioning on the task party and early-joining data parties. Unfortunately, this method tends to depreciate the late-coming data party if it shares some similar features with the early-coming ones. Consider an extreme case where two data parties $d$ and $d'$ have exactly the same set of features, \emph{i.e.}, $\bm {X}_{d} = \bm {X}_{d'}$. In this example, while $d$ and $d'$ should have the same data value to the task party, CMI will assign all the credits to the prior estimated data party and zero to the latter. In brief, an ideal data valuation method for VFL with multiple data parties should be able to incorporate the parties' correlations but be insensitive to their estimation order.

%we should expect that the estimated value of a data party should be insensitive to the estimation order of parties.

%While CMI can measure the data value via quantifying the coupling tightness between features and task labels, it cannot be applied directly to the VFL scenarios where multiple data parties are available. To understand this, we assume data parties enter the VFL system orderly and data valuations are thus launched in sequence by the task party. As a result, for any late-coming data party, its data value tends to depreciate for there might exist some early-coming data parties that share some similar features with the late-coming one. Consider an extreme case where two data parties $d$ and $d'$ have exactly the same set of features, \emph{i.e.}, $\bm {X}_{d} = \bm {X}_{d'}$. In this example, $d$ and $d'$ are supposed to have the same data value to the task party, whereas CMI will assign all the credits to the prior estimated data party and zero to the latter. In light of this, we should expect that the estimated value of a data party should be insensitive to the estimation order of parties.

%In general, successively measuring CMI of each data party likely undervalue the latterly estimated data parties as we have:
	%\begin{equation}
	%	I(\bm {\bar X}_j;Y|\bm X, \bm {\bar X}_{j-1}) \le I(\bm {\bar X}_j;Y|\bm X)
%\end{equation}}
%The assessed importance of a feature is dependent on the selected ones.

%While CMI works well for the one data party valuation, directly applying it to the multiple data parties scenario will cause certain problem. An intuitive extension of CMI to multi-party data valuation is that a party can calculate the CMI given the features already included in the federated parties. For example, the first joined data party $u_i$ with the features $\bm {\bar X}_i$ can calculate the CMI same as the two-party process, i.e., $I(\bm {\bar X}_i;Y|\bm X)$, while the second joined data party $u_j$ needs to compute CMI given both $\bm X$ and $\bm {\bar X}_i$, i.e., $I(\bm {\bar X}_j;Y|\bm X, \bm {\bar X}_i)$. Note that,
%\begin{equation}
%	I(\bm {\bar X}_j;Y|\bm X, \bm {\bar X}_i) \le I(\bm {\bar X}_j;Y|\bm X)
%\end{equation}
%That is, if there are more parties in the federation, the CMI of a new joined party will become smaller, thus discouraging the new parties from joining the federation. Hence, directly computing CMI in the multi-party data valuation scenario will not be a good choice.

To achieve an order-irrelevant estimation, 
we refer to the game theory of multiple parties~\cite{shapley1953value} and average the marginal values of a game party by considering all possible game-joining orderings of the parties. Let $\bm{\mathcal D}$ denote the set of all parties in a game, and $D\subseteq \bm{\mathcal D}$ denote the set of parties that have joined the game and yielded the game value $val(D)$. Then for a new party $d$, its game value can be estimated by 
%To achieve the order-irrelevant estimation, Shapley value in game theory averages the marginal values of a game party by considering all possible game-joining orderings of parties  \cite{shapley1953value}:
%
%we draw on the Shapley value from the game theory \cite{shapley1953value}. In particular, Shapley value In other words, compute a fair distribution of values over multiple parties we build a Shapley value based CMI metric, called \textit{Shapley-CMI}, to valuate multiple data parties in a collaborative task
%To alleviate the above pitfall, we build a Shapley value based CMI metric, called \textit{Shapley-CMI}, to valuate multiple data parties in a collaborative task. In particular, Shapley value is a classical metric to compute a fair distribution of values over multiple parties from the game theory \cite{shapley1953value}. The basic idea is, for the parties in the game, all the possible game-joining sequences, i.e., all the permutations of the parties, are enumerated and the Shapley value is the average of the marginal contribution of a party at each permutation,
%\begin{equation}
%	\varphi_j = \sum_{S \subseteq \{D_1, ..., D_l\} \setminus \{ D_j\} }\frac{|S|!(l-|S|-1)!}{l!} (val(S \cup \{D_j\})-val(S))
%\end{equation}
\begin{equation}\label{eq:value2}
	\varphi_d = \sum_{D \subseteq \bm{\mathcal D} \setminus \{ d\} }\frac{|{D}|!(|\bm{\mathcal D}|-|{D}|-1)!}{|\bm{\mathcal D}|!}\left(val({D} \cup \{d\})-val({D})\right).
\end{equation}
Eq.~\eqref{eq:value2} approximates the expected marginal improvement of party $d$ to a game by taking the average on all possible combinations of $D$. The combinatorial numbers in the equation are used to characterize the weight of each combination. Specifically, given the data parties in $D\cup\{d\}$, the possible number of permutations with $d$ as the last-in party is $|D|!$, and the possible number of permutations for $(|D|+1)$ parties selected from $\bm{\mathcal{D}}$ is $|\bm{\mathcal{D}}|!/(|\bm{\mathcal{D}}|-|D|-1)!$. Hence, the occurrence probability of $D\cup\{d\}$ with $d$ as the last-in party is $|D|!(|\bm{\mathcal{D}}|-|D|-1)!/|\bm{\mathcal{D}}|!$, which is right the weight of marginal improvement by $d$ in Eq.~\eqref{eq:value2}. 

We then go back to the VFL scenario. From the perspective of data valuation, we can apply CMI to measure the marginal value of a data party $d$ to the task party given a party joining-order, and compute an average marginal value by enumerating all data party orders to valuate the party $d$. In other words, the CMI metric is adopted as the game value $val(\cdot)$ in Eq.~\eqref{eq:value2}, that is
\begin{equation}\label{eq:val}
	val(D) = I(\bm{X}_D;Y_t| \bm{X}_t),
\end{equation}
where $\bm {X}_D$ denotes the set of features of all the data parties in $D$. Regarding the chain rule, we can easily have
\begin{equation}\label{eq:chain}
	I(\bm{X}_d;Y_t|\bm{X}_D \bm{X}_t) = I(\bm{X}_d\bm{X}_D;Y_t| \bm{X}_t) - I(\bm{X}_D;Y_t| \bm{X}_t).
\end{equation}
As a result, by replacing the $val(D)$ in Eq.~\eqref{eq:value2} by the $val(D)$ in Eq.~\eqref{eq:val} and using the chain rule in Eq.~\eqref{eq:chain}, we finally have the data value of $d$ in the case of multiple data parties as  
\begin{equation}
	\varphi_d = \sum_{D \subseteq \bm{\mathcal D} \setminus \{d\} }\frac{|D|!(|\bm {\mathcal{D}}|-|D|-1)!}{|\bm {\mathcal{D}}|!} I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t).
	\label{eq:shapley-cmi}
\end{equation}
%Note that, as the task party $u$ holds her own feature set $\bm X$, calculating CMI should also take $\bm X$ into consideration.
We call $\varphi_d$ in Eq.~\eqref{eq:shapley-cmi} as \emph{Shapley-CMI} to recognize the influence of Shapley's game theory~\cite{shapley1953value} to this metric. It is easy to note that when there is only one data party $d$, we have $D=\emptyset$ and $\bm{\mathcal{D}}=\{d\}$, and $\varphi_d$ in Eq.~\eqref{eq:shapley-cmi} thus reduces to $I(\bm {X}_d;Y_t|\bm X_t)$, which is consistent with the CMI metric for one data party. As a result, Shapley-CMI is a general-purpose metric for data valuation of VFL with an arbitrary number of data parties. 

\emph{Remark}.~To our best knowledge, Shapley-CMI is the first task-specific but model-free data valuation metric for multi-party VFL tasks. Inherited from CMI, Shapley-CMI is task-specific by incorporating task labels. It is also a model-free metric that can value data of multiple parities without running specific models. Finally, Shapley-CMI is a sound metric that takes the game behavior of different parties into consideration. These merits make Shapley-CMI a promising tool for data pricing prior to data transactions, which is particularly important to fostering legitimate data markets, a considered trillion-level business in the digital economy era~\cite{chui2014government}.  

In what follows, we highlight some properties possessed by Shapley-CMI, which ensures its interpretability and validity. 

\textsc{Property 1} \textbf{(Additivity)}: The sum of all the data parties' Shapley-CMI equals the CMI between the task label and all the data parties' features given the task party's features, \emph{i.e.},
\begin{equation}
\sum_{d\in \bm{\mathcal D}} \varphi_d = I(\bm {X}_{\bm{\mathcal{D}}}; Y_t|\bm {X}_t).
\end{equation}

\textsc{Property 2} \textbf{(Missingness)}: If a party's features are useless in predicting $Y_t$, then its Shapley-CMI value equals zero, \emph{i.e.},
\begin{equation}
    \varphi_d = 0, \text{if } I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t) = 0, \forall D \subseteq \bm{\mathcal D} \setminus \{d\}.
\end{equation}

\textsc{Property 3} \textbf{(Consistency)}: Two parties with the features of the same contribution have the same Shapley-CMI values, \emph{i.e.},
\begin{equation}
\varphi_d = \varphi_{d'}, \text{if } I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t) = I(\bm { X}_{d'};Y_t|\bm {X}_D \bm X_t), \forall D \subseteq \bm{\mathcal D} \setminus \{d,d'\}.
\end{equation}

%Apparently, the above properties are all required for a VFL data valuation metric to ensure its interpretability and validity.

%\textsc{Theorem 1} \textit{Shapley-CMI equals CMI when there is only one data party.}

%\textbf{Remark on Novelty}. %Regarding our Shapley-CMI metric, the most related work is SHAP (SHapley Additive exPlanations), which was proposed to explain the importance of each feature in a prediction model~\cite{Lundberg2017}. While our metric and SHAP are both inspired by the Shapley value in the game theory \cite{shapley1953value}, SHAP scores can only be computed if a certain prediction model has already been trained. That is, the SHAP scores are model-dependent.
%To the best of our knowledge, our proposed Shapley-CMI is the first task-specific and model-free data valuation metric. We note that a model-free data valuation method would be more favorable for VFL as a VFL task may adopt an arbitrary model and need the data valuation before model training. %In FL, data valuation should be done before model training, since a task party may use the data valuation results to decide the participants of its VFL task.
%We also highlight that Shapley-CMI is a general metric and contributes toward the data valuation research area.

\subsection{Dual-server-aided Federated Computation for Shapley-CMI}
\label{sub:fed_computation_cmi}
In general, Shapley-CMI can be directly computed if the data from various parties can be gathered. This, however, is not true in VFL contexts where all the parties keep their data private. Therefore, we propose a novel \emph{dual-server-aided private set intersection} (PSI) mechanism to attain privacy-preserving Shapley-CMI computation. Subsequently, we first analyze how federated Shapley-CMI computation is related to PSI. We then elaborate on how our novel dual-server-aided PSI mechanism can boost the computation of Shapley-CMI in VFL.

%describe how to calculate CMI to valuate the contribution of a data party in a VFL task given the task party without revealing any party's raw data. We then extend the mechanism to Shapley-CMI for the VFL tasks with multiple data parties.

%In the last subsection, we have elaborated on the Shapley-CMI metric and its key properties. In this subsection, we will continue describing how to calculate Shapley-CMI in the federated learning setting without revealing any party's information. We first illustrate how to compute CMI for two-party data valuation, and then extend the mechanism to Shapley-CMI for multi-party.

\subsubsection{Analysis of Federated Shapley-CMI Computation}
Here, we analyze the key of the federated Shapley-CMI computation problem. Without loss of generality, we assume the VFL task has multiple data parties. Following the maximum likelihood method in Eq.~\eqref{eq:cmi_ml2}, we can rewrite $I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t)$ in Eq.~\eqref{eq:shapley-cmi} as
\begin{equation}
	I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t) \nonumber
\end{equation}
\begin{equation}
	= \sum_{\bm {x}_d, \bm {x}_D,  \bm x_t, y_t} \hat{p}(\bm {x}_d \bm {x}_D \bm {x}_t y_t) \log \frac{\hat p(\bm {x}_d y_t|\bm x_t \bm {x}_D)}{\hat p(\bm {x}_d|\bm x_t \bm {x}_D)\hat p(y_t|\bm {x}_t \bm {x}_D)}
	\label{eq:CMI_multi}
\end{equation}
\begin{equation}
    = \frac{1}{n} \sum_{\bm {x}_d, \bm {x}_D,  \bm x_t, y_t} N(\bm {x}_d \bm {x}_D \bm {x}_t y_t) \log \frac{N(\bm {x}_d \bm {x}_D \bm {x}_t y_t)\sum_{\bm {x}_d' \in\mathcal{X}_d, y'_t \in \mathcal{Y}_t} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t')}{\sum_{y_t'\in \mathcal{Y}_t} N(\bm {x}_d \bm {x}_D\bm {x}_t y'_t)\sum_{\bm {x}_d' \in \mathcal{X}_d} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t)},
	\label{eq:CMI_multi_v2}   
\end{equation}
where $D$ denotes the set of parties that joined the VFL task ahead of the party~$d$, and $\bm {x}_D = \{\bm {x}_{d'} | d' \in D\}$ is a set of stacked features from the parties in $D$. In this vein, the problem of federated Shapley-CMI computation can be converted to calculating the \textit{cardinality of intersection} among various parties without gathering or revealing any party's raw data, \emph{i.e.}, 
\begin{equation}
    \label{eq:con_prob_expand}
    N(\bm{x}_d \bm{x}_D \bm{x}_t y_t) = \left|\left\{i|\langle\bm{x}_{t[i]}, y_{t[i]}\rangle = \langle\bm x_t, y_t\rangle\right\}\bigcap_{d'\in D\cup\{d\}}\left\{i|\bm {x}_{d'[i]}=\bm {x}_{d'}\right\}\right|,
\end{equation}
%where $i$ denotes the the $i$-th data sample whose feature values are $\langle\bm{x}_t,y_t\rangle$, $\bm{x}_d$, or $\bm{x}_D$, respectively. 
where $i$ denotes the $i$-th data sample whose feature values in the task party~$t$, data party~$d$ and data parties $D$ are $\langle\bm{x}_t,y_t\rangle$, $\bm{x}_d$, and $\bm{x}_D$, respectively. When there is only one data party $d$, \emph{i.e.}, $D=\emptyset$, the components $\sum_{\bm {x}_d' \in\mathcal{X}_d, y'_t \in \mathcal{Y}_t} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t')$ and $\sum_{\bm {x}_d' \in \mathcal{X}_d} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t)$ in Eq.~\eqref{eq:CMI_multi_v2} respectively degenerate to $N(\bm {x}_t)$ and $N(\bm {x}_t y_t)$, which can be computed within the task party only. 

\begin{comment}
\color{blue}

%\textbf{Federated CMI computation for one data party}.
Firstly, we analyze the federated Shapley-CMI computation problem for the VFL tasks with one data party and one task party. \color{black} Recall that $\hat p(y_t|\bm x_t)$, $N(\bm {x}_d \bm {x}_t y_t)$, $\hat p(\bm {x}_d y_t|\bm x_t)$ and $\hat p(\bm {x}_d|\bm x_t)$ are the four key components of the CMI computation with the maximum likelihood estimation (Eq.~\ref{eq:cmi_ml}). %Actually, while $\bm x$ and $\bm {\bar x}$ includes multiple features, we can see them as a \textit{combinatorial} feature. For example, suppose we have two binary features, then we can see them as one four-class combinatorial feature.\footnote{A combined feature may be very high-dimensional, which leads to other challenges in computing CMI. We will discuss this in Sec.~\ref{sub:approximate_CMI}.} Besides,
While the task party can easily compute $\hat p(y_t|\bm x_t)$ with its own data, it is challenging to compute $N(\bm {x}_d \bm {x}_t y_t)$, $\hat p(\bm {x}_d y_t|\bm x_t)$ and $\hat p(\bm {x}_d|\bm x_t)$ directly, as the data  are separately preserved by the task party (i.e., $\bm {x}_t,\ y_t$) and data party (i.e., $\bm {x}_d$). Moreover, we have the following equations:
\begin{align}
	\hat p(\bm {x}_d|\bm x_t) &= \sum_{y_t \in \mathcal Y_t} \hat p(\bm {x}_d y_t|\bm x_t) \\
	\hat p(\bm {x}_d y_t|\bm x_t) &= \frac{\hat p(\bm {x}_d \bm x_t y_t)}{\hat p(\bm x_t)}=
\frac{N(\bm {x}_d \bm {x}_t y_t)}{N( \bm {x}_t)}
\end{align}
Hence, we can re-write the computation of CMI (Eq.~\ref{eq:cmi_ml}) as,
\begin{equation}
	\hat I(\bm {X}_d;Y_t| \bm X_t) =\frac{1}{n} \sum_{\bm {x}_d} \sum_{\bm {x}_t} \sum_{y_t} N(\bm {x}_d \bm {x}_t y_t) \log \frac{N(\bm {x}_d \bm {x}_t y_t)}{\sum_{y_t'\in \mathcal Y_t}N(\bm {x}_d \bm {x}_t y_t') \hat p(y_t|\bm {x}_t)}
	\label{eq:cmi_ml_2}
\end{equation}
Then, the challenge of federated CMI computation turns to calculate $N(\bm {x}_d \bm {x}_t y_t)$ with no raw data transmission between the task and data parties:
\begin{equation}
 N(\bm {x}_d \bm {x}_t y_t) = |\{i|  \bm {x}_{d[i]} =  \bm {x}_d\}\cap \{i'|  \langle \bm x_{t[i']}, y_{t[i']} \rangle = \langle \bm x_t, y_t \rangle\}|
	\label{eq:con_prob_expand}
\end{equation}
where $i\in \mathcal I$ or $i' \in \mathcal I$ is a data sample, $\bm {x}_{d[i]}$ denotes the feature value vector of sample $i$ stored in data party $d$, $\bm { x}_{t[i']}$ and $y_{t[i']}$ respectively stand for the feature value vector and task label of sample $i'$ owned by task party $t$, and $N(\bm {x}_d \bm {x}_t y_t)$ essentially computes the number of samples who have data $\langle \bm {x}_d, \bm x_t, y\rangle$. In other words, $N(\bm {x}_d \bm {x}_t y_t)$ calculates the \textbf{cardinality of the intersection set} between the samples who have $\bm {x}_d$ in the data party and the samples who present $\langle \bm x_t, y_t\rangle$ in the task party.


%\color{blue} This problem, i.e., computing set intersection among various parties without revealing their raw data, is often denoted as \textbf{Private Set Intersection (PSI)} in literature \cite{Kamara2014ScalingPS}. Next, we illustrate that the general Shapley-CMI computation among multiple data parties can also be converted to PSI.

%In this vein, the task of $ N(\bm {\bar x} \bm {x} y)$ computation in VFL basically relates to the widely studied \textbf{private set intersection} (PSI) problem in the multi-party secure computation (MPC) area. Next, we first introduce the typical PSI solution and analyze its deficiency to our problem; we then propose a novel \textit{dual-server-aided PSI size computation} mechanism to attain privacy-preserving CMI computation for VFL task.
\color{black}

\vspace{+.5em}
%\textbf{Federated Shapley-CMI computation for multiple data parties}.
We furthermore analyze the federated Shapley-CMI computation for a VFL task with multiple data parties and rewrite $I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t)$ in Eq~\ref{eq:shapley-cmi} as:
\begin{align}
	&I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t) \nonumber \\ &= \frac{1}{n} \sum_{\bm {x}_d, \bm {x}_D,  \bm x_t, y_t} N(\bm {x}_d \bm {x}_D \bm {x}_t y_t) \log \frac{\hat p(\bm {x}_d y_t|\bm x_t \bm {x}_D)}{\hat p(\bm {x}_d|\bm x_t \bm {x}_D)\hat p(y_t|\bm {x}_t \bm {x}_D)}
	\label{eq:CMI_multi} \\&= \frac{1}{n} \sum_{\bm {x}_d, \bm {x}_D,  \bm x_t, y_t} N(\bm {x}_d \bm {x}_D \bm {x}_t y_t) \log \frac{N(\bm {x}_d \bm {x}_D \bm {x}_t y_t)\sum_{\bm {x}_d' \in\mathcal{X}_d, y'_t \in \mathcal{Y}_t} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t')}{\sum_{y_t'\in \mathcal{Y}_t} N(\bm {x}_d \bm {x}_D\bm {x} y')\sum_{\bm {x}_d' \in \mathcal{X}_d} N(\bm {x}_d' \bm {x}_D \bm {x}_t y_t)} \label{eq:CMI_multi_v2}
\end{align}
where $D$ denotes the set of parties that joined in the VFL task before the party $d$ and $\bm {x}_D = \{\bm {x}_{d'} | d' \in D\}$ is a set of features from the parties in $D$. In this vein, the problem of federated Shapley-CMI computation can be converted to calculate the \textit{cardinality of intersection} among various parties given a VFL task (i.e.,  $N(\bm {x}_d \bm {x}_D \bm {x}_t y_t)$) without gathering or revealing any party's raw data.
\end{comment}

\subsubsection{Analysis of Potential Solution}
Secure multi-party computation (MPC) protocols are one class of solutions that can support joint computations of data from multiple parties but reveal nothing other than the computational results to any of the parties. \emph{Private Set Intersection} (PSI) is a specific MPC application, which allows each party to learn the intersection of item sets among various parties. The PSI result can make each party easily calculate the intersection cardinality for Shapley-CMI computation, whereas it would also violate the privacy requirement of VFL. Let suppose that a data party $d$ has a set of samples with features $\bm{x}_d=\langle 1, 0 \rangle$, and a task party $t$ owns a set of samples with label $y_t=1$. PSI could be applied to let $d$ and $t$ acquire their intersection samples whose features and label are respectively $\bm{x}_d=\langle 1, 0 \rangle$ and $y_t=1$ for intersection cardinality computation; nevertheless, the intersection samples' label information $y_t=1$ is exposed from $t$ to $d$, and their feature information $\bm {x}_d=\langle 1, 0 \rangle$ is leaked from $d$ to $t$, which should be prohibited in VFL tasks.


%Secure multi-party computation (MPC) protocols are one class of solutions that can support joint computations of data from multiple parties but reveal nothing other than the computational results to any of the parties. As a typical application of MPC, \emph{Private Set Intersection} (PSI) computes and notifies the parties with the \emph{elements} in the intersection set of various parties~\cite{Kamara2014ScalingPS}. However, allowing the parties to learn the elements of the intersection set may violate the privacy requirement of VFL. Suppose one data party $d$ has a set of samples with features $\bm{x}_d=\langle 1, 0 \rangle$, and the task party $t$ owns a set of samples with label $y_t=1$. If the parties $d$ and $t$ learn the samples of their intersection set, then the samples' label $y_t=1$ is exposed to the data party, and their features $\bm {x}_d$ are leaked to the task party.

A few recent studies design MPC protocols to compute arbitrary functions (e.g., cardinality) over the intersection set but avoid disseminating its elements to attendees for information protection. Most of these methods, however, can only operate on MPC tasks with \emph{two} parties~\cite{Le2019TwopartyPS}, and thus a new MPC protocol is desired to compute the cardinality of the intersection set of \emph{multiple} parties for data valuation in VFL tasks. It is worth noting that designing an MPC protocol for secured intersection cardinality computation is more challenging than that for the intersection element computation~\cite{Le2019TwopartyPS}. The essential difficulty lies in how each party discriminates the veracity of its received intersection cardinality when there exist malicious participants in MPC. We will articulate the difficulties in the sections to follow.

In summary, we require a \emph{secure}, \emph{multi-party}, \emph{PSI} \emph{cardinality} computation mechanism for federated Shapley-CMI calculation, so that each party can obtain an undisputed result about the cardinality of various parties' intersection without sharing any raw data.


\subsubsection{Multi-party PSI Cardinality Computation with Semi-honest Server}
Server-aided and serverless solutions are two typical classes of MPC solutions. In general, server-aided MPC solutions are more efficient in large-scale computations, which are deemed as the typical scenario in real-life VFL practices~\cite{Kamara2014ScalingPS,Le2019TwopartyPS,Bogetoft2009SecureMC}. For example, the commercial VFL platform FDN (federated data network)\footnote{https://fdn.webank.com/} is required to support millions of samples. We adopt the server-aided strategy in this work accordingly. Specifically, we first propose a simple and efficient solution based on a \emph{semi-honest} aided server that would abide by the designed protocol. We then enhance the solution in the subsequent section to defend against \emph{untrustful} servers that may perform maliciously.

%compute the size of the intersection set between the samples with $\langle \bm {\bar x}, \bm x, y\rangle$ in task party and the samples with $\bm \bar{x}$ in data party, i.e., $N(\bm {\bar x} \bm {x} y)$.

%Our proposed mechanism is built based on untrusted third-party servers, belonging to the type of server-aided MPC solutions \cite{Kamara2014ScalingPS,Le2019TwopartyPS}. We choose the server-aided solution because it is the most efficient PSI solution up to date as far as we know,  which can run on billions of data points \cite{Kamara2014ScalingPS,Le2019TwopartyPS}. Furthermore, server-aided techniques have successfully been deployed in practice for multi-party secure computation \cite{Bogetoft2009SecureMC}, which indicates the practicability.
%Moreover,  same as prior research \cite{Kamara2014ScalingPS,Le2019TwopartyPS}, the two servers in our mechanism do not need to be \textit{trusted}; as long as the servers do not collude with others, then the mechanism can run safely (we will prove it later). %Note that, before data valuation, we assume that the task party and the data party have already synchronized their common data sample IDs with a certain data alignment method in any VFL protocol~\cite{Cheng2019SecureBoostAL}.
%Let assume that the data sample Ids on the task party and the data party have been synchronized in advance. Then, $N(\bm {\bar x} \bm {x} y)$ can be computed with an aided \textit{semi-honest} server (namely \textit{computation server}) by the following steps~\cite{Kamara2014ScalingPS}:

%\vspace{+.5em}
%\textbf{PSI Cardinality Computation with Semi-honest Server}


Basically, if we have a \emph{semi-honest} third-party server, we could refer to some PSI protocols to let the server collect encrypted sample sets from all parties and perform secure intersection computations~\cite{Kamara2014ScalingPS}. While PSI likely leads to information leakage by revealing the computed intersection to all parties, we only return the cardinality of intersection to each party instead for data protection. Detailed steps are as follows.
%can let this server do intersection computation and. All the parties precede transmitting sample IDs to the server with the encryption by an agreed scheme, thus the original sample IDs cannot be re-identified by the server. Detailed steps are as follows.


%Suppose we leverage a \emph{semi-honest} third-party server to collect the encrypted sample sets from all parties and do the intersection operation. All the parties precede transmitting sample IDs to the server with the encryption by an agreed scheme, thus the original sample IDs cannot be re-identified by the server. Detailed steps are as follows.

\begin{itemize}
\item[] \textbf{Preparation.} \textit{All the data parties and the task party agree on the same encryption scheme and encrypt their sample IDs, so that the original sample IDs cannot be re-identified by the server.}

\item[] \textbf{Step 1.} \textit{All the parties send their own encrypted ID sets to a semi-honest computation server for intersection computation.}

\item[] \textbf{Step 2.} \textit{The server computes the intersection of all the received ID sets and then returns its cardinality to all the parties.}
\end{itemize}

This procedure is simple and effective, only if the computation server is semi-honest and will not falsify the result.

\subsubsection{Multi-party PSI Cardinality Computation with Untrustful Server}
\label{sec:mp-PSI}
In practice, the computation server could be untrustful and may mislead the task party's data valuation maliciously. For instance, if the task party's set cardinality is $n_t$, the task party barely discriminates the server's malicious report with any forged intersection cardinality $\hat n\ (\le n_t)$.
To deal with this, in what follows, we propose a novel \emph{dual-server-aided PSI cardinality computation mechanism}, as shown in Fig.~\ref{fig:psi_computation_framework}.

\begin{figure}
	\includegraphics[width=\linewidth]{./fig/framework.pdf}
	\vspace{-2em}
	\caption{Dual-server-aided PSI cardinality computation mechanism.}
	\label{fig:psi_computation_framework}
\vspace{-1em}
\end{figure}

We first introduce a new \emph{validation server} that incorporates an \emph{ID Duplication} mechanism to detect the computation server's malicious report with a non-zero value. Basically, the ID duplication mechanism requires the parties to generate $q$ different encryption IDs for each sample ID, and let the computation server operates on all the encryption IDs. Note that the computation server is ignorant but the validation server is informed about how many and which encryption IDs correspond to the same sample IDs. The computation server respectively sends the encryption IDs of intersection set to the validation server and feeds back the intersection cardinality to the parties. Following the widely accepted assumption in server-aided MPC that the validation server will not collude with the computation server\footnote{We can leverage the two servers in two competitive cloud services (\emph{e.g.}, Microsoft Azure and Amazon Web Services) and use contracts to regularize such collusion behaviors~\cite{Bogetoft2009SecureMC,Kamara2014ScalingPS}.}, we can count on the validation server to detect the computation server's malicious behavior by mapping its received encryption IDs back to the sample IDs. In principle, if the computation server is veracious, the validation server would obtain $q$ duplicates for each  sample ID; otherwise, the computation server may be regarded malicious. If the computation server intends to successfully deceive with a forged intersection cardinality $\hat n$, it needs to correctly link each of the $\hat n$ sample IDs to its $q$ encryption IDs. Without knowing the exact mappings between the samples and their encryption IDs, it is nearly impossible for the computation sever especially when $q$ is large.



%We first introduce a new \emph{validation server} that incorporates an \emph{ID Duplication} mechanism to detect the computation server's malicious report with a non-zero value. Basically, the ID duplication mechanism requires the parties to generate $q$ different encryption IDs for each sample ID, and let the computation server operates on all the encryption IDs. Note that the computation server is ignorant but the validation server is informed about how many and which encryption IDs correspond to the same sample IDs. The computation server respectively sends the encryption IDs of intersection set to the validation server and feeds back the result of intersection cardinality to the parties. Following the widely accepted assumption in server-aided MPC that the validation server will not collude with the computation server\footnote{We can leverage the two servers in two competitive cloud services (\emph{e.g.}, Microsoft Azure and Amazon Web Services) and use contracts to regularize such collusion behaviors~\cite{Bogetoft2009SecureMC,Kamara2014ScalingPS}.}, we can count on the validation server to detect the computation server's malicious behavior if the encryption IDs of the intersection set cannot be mapped back to $q$ duplications of the sample IDs. In other words, if the computation server intends to deceive the parties by a forged number $\hat n$, it needs to identify correctly the $q$ encryption IDs of $\hat n$ sample IDs, which is very difficult especially when $q$ is large, as it does not know the mappings of sample IDs and encryption IDs.

Unfortunately, the validation server is yet incompetent to discriminate the credibility of the computation server's result with a zero intersection cardinality. Besides, after running several rounds of intersection operations, untrustful servers could probably learn the feature distribution of data, which brings exposure risks in practice. To address these issues, we enhance the PSI cardinality computation with a \emph{randomized adversarial data augmentation} method. Simply speaking, this method produces a random number $n_r$ of adversarial data samples shared by all the parties and mixes them with real samples before computation. Then, the computed result of intersection cardinality should be a number no less than $n_r$ but larger than zero. The difference between the computed intersection cardinality and $n_r$ is the clear cardinality result. In other words, the parties could easily identify the computation server's malicious behavior if it returns a number less than $n_r$. 
%whose $\bm {\bar x}$, $\bm x$ and $y$. To remove the possibility of zero PSI cardinality, these random samples will cover all the feature value combinations. These random data samples' $\langle ID, \bm {\bar x}, \bm x, y \rangle$ are shared among all the parties but not exposed to the untrustful servers. Then, all the $n$ real data samples and $n_r$ random data samples together constitute the total data sample set. %Afterward, all the parties can safely send their data samples to the computation server for PSI size calculation, as the server cannot learn the real private feature distributions. Finally, all the parties obtain the clear cardinality result by subtracting the number of random adversarial data samples (i.e., $n_r$) from the cardinality result returned by the computation server.

Besides, the adversarial data samples would protect the real feature distribution from being learned. % we should not employ too many randomized data samples. 
More specifically, if we generate more adversarial data samples, the server-observed feature distribution will be closer to that of the adversarial samples but deviate more from the real one. Nevertheless, more adversarial data samples will incur a higher data transmission workload. As a result, we should carefully set the number of adversarial data samples to strike a balance between the risks from malicious attacks and the costs of data transmissions in practice.

\begin{algorithm}[t!]
	\footnotesize
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{
		$\bm D$: data parties, each data party $d$ with features ${\bm X}_d$;\\
		$T$: task party with features $\bm X_t$ and label $Y_t$.
	}
	\Output{$\bm \varphi = \{\varphi_1, \varphi_2,...\}$: Shapley-CMI values for all the data parties.}
	$\pi \leftarrow all\_permutations(\bm D) $ \;
	$\bm \varphi = [0] * |\bm D| $\;
	\For{$O \in \pi$}{
		$D = []$\;
		\For{$k \in [1,2,...,|\bm D|]$}{
			$d = O[k]$ \tcp*{data party $d$}
			\tcc{compute CMI with dual-server-aided PSI mechanism}
			$\bm \varphi[d] += I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t)$\;
			$D.\textit{append}(d)$\;
		}
	}
	$\bm \varphi = \bm \varphi/|\pi|$\;
	%\Return $\bm \varphi$\;
	\caption{Federated Computation of Shapley-CMI}
	\label{alg:shapley-cmi}
\end{algorithm}

Algorithm~\ref{alg:shapley-cmi} illustrates the federated Shapley-CMI computation process. We describe the proposed protocol as follows.

\begin{itemize}
    \item[] \textbf{Preparation.} \textit{First, all the data parties and the task party make agreements on the same encryption scheme, the number of encryption IDs for each sample (i.e., $q$), and the random number of adversarial data samples (i.e., $n_r$). Then, each of the data parties (i.e., $d$ or $d'\in D$) and the task party extract the subset of targeted samples with certain data values (i.e., $\bm {x}_d$, $\bm {x}_{d'}$ or $\langle \bm {x}_t,y_t \rangle$), and accordingly produce $n_r$ adversarial sample IDs with the same values as the targeted samples. Furthermore, every party constitutes an encryption ID set by generating $q$ different encryption IDs for each of the targeted and adversarial samples. Finally, the validation server is informed with which $q$ encryption IDs correspond to the same sample ID.}

%All the data parties and the task party agree on a same encryption scheme, and use it to encrypt their data sample IDs. Besides, some new data sample IDs are generated randomly, shared among all the parties, and added to the total sample set. Then, each sample ID $i$ is duplicated for $m$ times, i.e., $\{i'|i'=dup(i, k), k=0,...,m-1\}$ where $dup()$ is the ID duplication function.\footnote{The $dup()$ function is defined to ensure that $dup(i_i,k_1) \not = dup(i_2, k_2)$ if $i_1 \not = i_2$ or $k_1 \not = k_2$. } Finally, the validation server is informed with whether two encrypted IDs are mapped to the same sample or not.

    \item[] \textbf{Step 1.} \textit{The data parties and the task party send their encryption ID sets to the computation server for intersection computation.}

    \item[] \textbf{Step 2.} \textit{The computation server computes the intersection ID set $\bm I_\textit{inter}$ and transmits it to the validation server (\emph{\textbf{Step 2.1}}); it meanwhile calculates the intersection cardinality $n_c = |\bm I_\textit{inter}|$ and feeds it back to the parties (\emph{\textbf{Step 2.2}}).}

    \item[] \textbf{Step 3.} \textit{The validation server checks whether the encryption IDs in $\bm I_\textit{inter}$ can be mapped to $\frac{|\bm I_\textit{inter}|}{q}$ samples with $q$ duplicates for each; %how many ($q$ or 0) encryption IDs of a sample exist in $\bm I_\textit{inter}$;
    If the answer is yes, it sends $n_v = |\bm I_\textit{inter}|$ to the parties; otherwise, it sends $-1$.}

    \item[] \textbf{Step 4.} \textit{The parties compare $n_c$ and $n_v$. If $n_c = n_v$, the intersection cardinality is $n_c/q - n_r$; otherwise, there must be certain malicious server behaviors.}
\end{itemize}

%Here, we elaborate on two key techniques of the mechanism to fight against servers' malicious behaviors.


%\textbf{\textit{ID Duplication}}. In the data preparation step, the mechanism duplicates all the sample IDs for $m$ times. With the ID duplication, if the computation server wants to maliciously report a wrong intersection cardinality, it has to correctly guess which $m$ encrypted IDs exactly correspond to one sample. For example, if the computation server wants to report the intersection cardinality as $\hat s$, it needs to find $\hat s$ samples with their duplicated $m$ IDs, i.e., a forged intersection set $\bm \hat I_{inter}$ including $m \hat s$ IDs exactly mapped to $\hat s$ different samples. As the computation server does not know how sample IDs are duplicated, it can hardly construct such a forged ID set. Note that the ID duplication results are exposed to the validation server, so the validation server can check that, for each ID in $\bm I_{inter}$ (sent by the computation server), whether its other $m-1$ duplicated IDs are also in $\bm I_{inter}$. The larger $m$ is, the more difficult that the computation server can successfully cheat the validation server by forging $\bm \hat I_{inter}$.






%\vspace{+.5em}
%\textbf{\textit{Randomized Data Augmentation}}. With the ID duplication method, there are still two potential risks: (i) the computation server can maliciously claim that there are no intersected IDs (i.e., the cardinality is 0), which is hard to check by the validation server as $\bm I_{inter} = \phi$; (ii) after running several rounds of intersection operations, untrustful servers can learn data samples' feature distribution, which may not be desirable in practice. To address these issues, we enhance the PSI mechanism with \textit{randomized data augmentation}. In particular, before computing Shapley-CMI, all the parties agree on generating $n_r$ new data samples whose $\bm {\bar x}$, $\bm x$ and $y$ are randomized. To remove the possibility of zero PSI cardinality, these random samples will cover all the feature value combinations. These random data samples' $\langle ID, \bm {\bar x}, \bm x, y \rangle$ are shared among all the parties but not exposed to the untrustful servers. Then, all the $n$ real data samples and $n_r$ random data samples together constitute the total data sample set. Note that after obtaining the PSI cardinality returned from the servers, all the parties need to subtract the intersection cardinality incurred by the random data samples. In general, if we generate more randomized data samples, the server-observed feature distribution will be closer to the random samples' feature distribution, thus deviating from the real one. Meanwhile, more randomized data samples will incur higher data transmission workload. In practice, we can trade off the random data sample number to achieve satisfactory protection with the affordable data transmission amount.



%In summary, the federated Shapley-CMI computation process is illustrated in Algorithm~\ref{alg:shapley-cmi}.


%which can also be addressed by the proposed dual-server-aided PSI. The slight difference is that there are multiple data parties (party $j$ and all the parties in $S$), while all the process can still follow Fig.~\ref{fig:psi_computation_framework}.

%We note that the data valuation by Shapley-CMI (Eq.~\ref{eq:shapley-cmi}) needs to enumerate every possible party-joining order. %(i.e., $N(\bm {\bar x}_j \bm {\bar x}_S \bm {x} y),  \forall \{D_j\}\cup S \subseteq \{D_1 ... D_l\}$), %(i.e., $\{D_j\}\cup S$ can be any subset of all the data parties),
%Hence, its computational complexity is $O(2^{l})$, where $l$ is the number of data parties. This may be tractable when $l$ is not large. %; however, it is hard to generalize to a large number of parties. In the next subsection, we illustrate some approximation Shapley-CMI computation methods to overcome the high computation overhead.



%\textbf{Remark on Novelty}. To the best of our knowledge, our work is the first one to design federated computation mechanisms for CMI (and further, for Shapley-CMI). In particular, we convert the CMI computation to the sub-problems of PSI size calculation, and propose a novel dual-server-aided PSI mechanism. Specifically, our mechanism is inspired by the server-aided mechanism \cite{Kamara2014ScalingPS}, which aims to obtain the elements of PSI. As we only need to know the PSI size, \cite{Kamara2014ScalingPS} cannot be directly applied. We emphasize that our dual-server-aided PSI mechanism can serve various tasks requiring PSI size calculation from multiple parties (not only CMI computation), which itself is a contribution toward the PSI research area.

\emph{Remark}.~To the best of our knowledge, this is the first work that designs a federated mechanism for CMI as well as Shapley-CMI computation. In particular, we first convert the federated CMI computation issue to the PSI cardinality calculation problem, %propose a novel dual-server-aided PSI mechanism. %Here, we highlight the novelty of our dual-server-aided PSI mechanism over literature. Specifically, The existing server-aided PSI mechanism \cite{Kamara2014ScalingPS} transfers the intersection elements to the parties against malicious servers, which may violate the data privacy regulation in VFL. While we only need to know the PSI cardinality,
and then propose a novel dual-server-aided mechanism to compute the multi-party PSI cardinality without leaking raw data from any parties. It should be emphasized that this mechanism can serve various tasks beyond CMI computation where a PSI cardinality calculation is required for multiple parties. In this light, it also contributes to the PSI research area.

\subsection{Practical Considerations}
\label{sub:approximate_CMI}

The Shapley-CMI metric and its secure multi-party PSI cardinality computation mechanism together constitute our FedValue framework. While FedValue is theoretically feasible for data valuation in VFL tasks, it still encounters some computational challenges in practice. First of all, the federated Shapley-CMI computation in Eq.~\eqref{eq:shapley-cmi} needs to enumerate every possible party-joining order, and hence its computational complexity is $O(2^{|\bm{\mathcal{D}}|-1})$, where $\bm{\mathcal{D}}$ is the set of all data parties. This indicates that the federated Shapley-CMI computation could be practically difficult for a VFL task with a large number of parties. Besides, if the parties' data are of very high dimensions, the maximum likelihood estimation of Shapley-CMI in Eq.~\eqref{eq:shapley-cmi} may not be reliable and thus the data valuation is likely imprecise~\cite{Brown2012}. Accordingly, we employ two practical techniques, \emph{i.e.}, \emph{Shapley sampling} and \emph{feature dimension reduction}, to address these practical issues in FedValue computation.
%In the next subsection, we illustrate some approximation Shapley-CMI computation methods to overcome the high computation overhead.

%So far, we have introduced our proposed Shapley-CMI data valuation metric and its federated computation mechanism. However, this valuation is built upon two assumptions: (1) the maximum likelihood estimation of the conditional probabilities in Eq.~\ref{eq:cmi_ml} are reliable and tractable, and (2) the number of parties is not large.

%The federated computation of Shapley-CMI may be practically difficult to a VFL task with a large number of parties. Besides, if the parties' data are of very high dimensions, the maximum likelihood estimation of CMI-computation (i.e., Eq.~\ref{eq:cmi_ml}) may not be reliable and thus the data valuation are likely imprecise~\cite{Brown2012}. Therefore, we intend to alleviate these practical computational issues by employing several practical techniques, including \textit{Shapley sampling}, \textit{feature dimension reduction}, and \textit{feature independence-assumed approximation}.


%In reality, both assumptions may fail: (1) the maximum likelihood estimation may not be reliable when the data dimensions of each party are high \cite{Brown2012}, and (2) there could be a large number of parties joining federated learning. We propose to alleviate these issues by the following techniques: \textit{feature independence-based CMI approximation}, \textit{feature dimension reduction},  and \textit{Shapley sampling}.








\subsubsection{Shapley Sampling}
\label{subsub:shapley_sampling}

%The original computation for Shapley-CMI (Eq.~\ref{eq:shapley-cmi}) needs to enumerate all the possible permutations of data parties, so the computation complexity becomes $O(l!)$, where $l$ is the number of data parties. This complexity can be quickly intractable when $l$ is large.

%In practice, we may use a sampling strategy to accelerate the Shapley-CMI computation  \cite{trumbelj2013ExplainingPM}.
Inspired by the prior Shapley value computation work~\cite{trumbelj2013ExplainingPM}, we leverage the approximation technique by sampling and enumerating a subset of permutations of data parties. %Inspired by prior work computing Shapley values \cite{trumbelj2013ExplainingPM}, we can use a sampling strategy. More specifically, instead of enumerating all the possible joining-orders, we can only sample a number of permutations of data party joining orders.
Specifically, a party $d$'s value $\hat \varphi_d$ is estimated by the average of CMI values given a sampled set of data party permutations. That is,
\begin{equation}
	\hat \varphi_d = \frac{1}{|\pi|} \sum_{\mathcal O \in \pi} I(\bm {X}_d;Y_t|\bm {X}_{\mathcal O_{d}} \bm X_t),
\end{equation}
where $\pi$ is a sampled set of permutations of data parties, $\mathcal O$ is a specific permutation of data parties in $\pi$, and $\mathcal O_{d}$ is the set of data parties that precede the party $d$ in $\mathcal O$. %Finally, a party $j$'s value $\hat \phi_j$ is computed as the average of values given a sampled set of permutations $\pi(l)$.

\subsubsection{Feature Dimension Reduction}
\label{subsubsec:feature_dimension_reduction}

Feature dimension reduction techniques are widely used in machine learning tasks, which can reduce the computation overhead and may even boost the learning performance \cite{fodor2002survey}. In our case, before calculating Shapley-CMI, all the parties can firstly run feature dimension reduction methods such as PCA~\cite{Martinez2001pca} and reduce the feature space to a controllable small scale, so that the Shapley-CMI computation can be accelerated. The PCA can be performed on each party independently and thus will not lead to any privacy leakage. Then, the proposed FedValue can work with the principal components obtained by PCA for data valuation in VFL. In the experiment, we will empirically investigate how feature dimension reduction impacts the Shapley-CMI computation results.

%\subsubsection{Feature Independence-assumed Approximation}
%\label{subsubsec:feature_indepence_appro}

%Feature independence (FI) is a common assumption for feature selection in machine learning tasks \cite{Brown2012}. Inspired by this, we propose a practical FI-assumed Shapley-CMI computation method for acceleration if a data party has a large number of features. Let first concern the case with only one data party who has a feature set $\bm {X}_d$. According to the chain rule~\cite{Brown2012}, we have
%\begin{equation}
%	I(\bm {X}_d;Y_t| \bm X_t)
%	= \sum_{k=1}^{|\bm {X}_d|} I(X_d^{(k)};Y_t|\bm X_t \cup \{X_d^{(1)},..., X_d^{(k-1)}\})
%	\label{eq:cmi_expansion}
%\end{equation}
%where $|\bm {X}_d|$ denotes the dimension of $\bm {X}_d$. On this basis, we assume that all the features in $\bm {X}_d$ are independent and rewrite Eq.~\ref{eq:cmi_expansion} as:
%\begin{equation}
%	I(\bm {X}_d;Y_t| \bm X_t)  = \sum_{k=1}^{|\bm {X}_d|} I(X_d^{(k)};Y_t|\bm X_t)
%	\label{eq:cmi_expansion_2}
%\vspace{-.5em}
%\end{equation}
%If the task party feature set $\bm X_t$ is high-dimensional, $I(X_d^{(k)};Y_t|\bm X_t)$ may still be hard to compute. By the chain rule, we have:
%\begin{equation}
%	I(X_d^{(k)};Y_t|\bm X_t) = I(X_d^{(k)}, \bm X_t;Y_t) - I(\bm X_t;Y_t)
%\end{equation}
%Let assume each feature in  $\bm X$ is independent. Then,
%\begin{equation}
%	I(X_d^{(k)};Y_t|\bm X_t) = \sum_{l=1}^{| \bm {X}_t|}I(X_d^{(k)}, X_t^{(l)};Y_t) - \sum_{l=1}^{|\bm X_t|}I(X_t^{(l)};Y)
%\end{equation}
%With the above assumptions in mind, we can approximate $I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t)$ for the Shapley-CMI calculation when there are more than one data party by:
%\begin{equation}
%	I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t) = \sum_{k=1}^{|\bm X_d|} I({X}_d^{(k)};Y_t|\bm {X}_{D} \bm X_t)
%\end{equation}
%and,
%\begin{align}
%	& I({X}_d^{(k)};Y_t|\bm {X}_{D} \bm X_t) = I({X}_d^{(k)} \bm {X}_{D} \bm X_t;Y_t) - I(\bm {X}_{D} \bm X_t;Y_t) \\
%	= & \sum_{k_1=1}^{|\bm X_{d_1}|}\sum_{k_2=1}^{|\bm X_{d_2}|}...\sum_{k_{|D|}=1}^{|\bm X_{d_{|D|}}|} I({X}_d^{(k)} {X}_{d_1}^{(k_1)} {X}_{d_2}^{(k_2)} ... {X}_{d_{|D|}}^{(k_{|D|})}\bm X_t;Y_t) \nonumber \\ & - \sum_{k_1=1}^{|\bm X_{d_1}|}\sum_{k_2=1}^{|\bm X_{d_2}|}...\sum_{k_{|D|}=1}^{|\bm X_{d_{|D|}}|} I({X}_{d_1}^{(k_1)} {X}_{d_2}^{(k_2)} ... {X}_{d_{|D|}}^{(k_{|D|})} \bm X_t;Y_t) \label{eq:approx_1}\\
%	= & \sum_{k_1=1}^{|\bm X_{d_1}|}\sum_{k_2=1}^{|\bm X_{d_2}|}...\sum_{k_{|D|}=1}^{|\bm X_{d_{|D|}}|}\sum_{l=1}^{|\bm X_t|}  I({X}_d^{(k)} {X}_{d_1}^{(k_1)} {X}_{d_2}^{(k_2)}... {X}_{d_{|D|}}^{(k_{|D|})} X_t^{(l)};Y_t)\nonumber \\ &- \sum_{k_1=1}^{|\bm X_{d_1}|}\sum_{k_2=1}^{|\bm X_{d_2}|}...\sum_{k_{|D|}=1}^{|\bm X_{d_{|D|}}|}\sum_{l=1}^{|\bm X_t|} I({X}_{d_1}^{(k_1)} {X}_{d_2}^{(k_2)}... {X}_{d_{|D|}}^{(k_{|D|})} X_t^{(l)};Y_t) \label{eq:approx_2}
%\end{align}
%where $d_1, d_2, ..., d_{|D|}\in D$ are the data parties that joined in the task before the data party $d$; $|{\bm X}_{d_1}|, |{\bm X}_{d_2}|, ..., |\bm X_{d_{|D|}}|$ respectively denote the feature dimensions of the data parties in $D$; $|\bm X_t|$ is the feature dimension of the task party $t$. Eq.~\ref{eq:approx_1} approximates CMI by assuming the features of data parties independent, while Eq.~\ref{eq:approx_1} further assumes that task party features $\bm X_t$ are independent.

%Suppose there are $|D|$ data parties, each party is of $|\bm X_d|$ features, and the task party has $|\bm X_t|$ features. For simplicity, we assume that all the features are binary. Then, the original computation complexity of  $I(\bm {X}_d;Y_t|\bm {X}_D \bm X_t)$ is $O(2^{|\bm X_d|(|D|+1)+|\bm X_t|})$ as we take all the features in one party as a large combined feature. By making the feature independence assumption on all the data parties (Eq.~\ref{eq:approx_1}), the complexity is $O(|\bm X_d|^{|D|+1}2^{|D|+1+|\bm X_t|})$; by further assuming the feature independence assumption on the task party (Eq.~\ref{eq:approx_2}), the complexity is reduced to $O(|\bm X_t||\bm X_d|^{|D|+1}2^{|D|+2})$. Hence, if $|\bm X_d|$ and $|\bm X_t|$ are large, the approximation can accelerate the running speed significantly.

%\color{blue}
%It is worth noting that, while the FI assumption is widely considered in literature \cite{Brown2012}, realistic data may not satisfy it well. Hence, the practical FI approximation performance needs to be carefully assessed (our experiment also shows diverse approximation results for different datasets, details in Sec.~\ref{sub:value_quality}). In practice, if a data party holds many features, we suggest first using feature dimension reduction techniques (Sec.~\ref{subsubsec:feature_dimension_reduction}). Feature dimension reduction methods, e.g., PCA, would generate (roughly) independent features for each party; then, we can apply FI-assumed approximation on the reduced features if the feature number is still large.







==> VFLValue AIJ/problem.tex <==
\section{Problem Formulation}
\label{sec:problem}
%\textbf{Two-Party Data Valuation Problem for Vertical Federated Learning}. Suppose there are two parties, the task party $u$ holds a set of features $\bm X$ and a target label $Y$, and a data party $\bar u$ holds another set of features $\bm {\bar X}$.\footnote{The naming of `active' and `data' parties are borrowed from SecureBoost \cite{Cheng2019SecureBoostAL}.} How to quantify the value of $\bm {\bar X}$ in predicting $Y$?

%While the two-party VFL is a simple setting for VFL, it has already shown the effectiveness and practicality in real applications, and many VFL algorithms are currently designed only for two parties [][]. To this end, in this paper, we first focus on the two-party VFL case for data valuation. After elaborating on the two-party solution, we will also illustrate how to extend our solution to a case where more parties are included:
Generally speaking, a \textit{federated learning system} makes use of distributed data from a few parties to collaboratively learn a model while ensuring that each party keeps its raw data unexposed to other parties~\cite{yang2019federated}. In this work, we consider a \emph{vertical} federated learning context where a task party (who seeks for task-specific models) and a set of data parties (who can provide data for collaborative modelling) are involved.

\begin{definition}[Task Party]
    A task party ${t}$ holds a group of data samples with a set of features $\bm X_t$ and a task label $Y_t$. The set of sample IDs of $t$ is denoted as $\mathcal I_t$.
\end{definition}

%\textsc{Definition 1.} \textbf{\textit{Task party.}} A task party ${t}$ often holds a group of samples' data including a set of features $\bm X_t$ and a task label $Y_t$. Let use $\mathcal I_t$ to denote the sample IDs of the task party.

In practice, a task party can hardly train a satisfactory model with its self-owned limited data features. However, it can get improved by inviting some data parties with incentives to launch a VFL task.

\begin{definition}[Data Party]
    A data party $d$ has no target labels but can provide data samples with features ${\bm{X}_d}$ to predict the task label $Y_t$. The set of sample IDs of $d$ is denoted as $\mathcal{I}_d$. The set of all available data parties is denoted as $\mathcal{D}$.
\end{definition}

%\textsc{Definition 2.} \textbf{\textit{Data party.}} A data party $d$ usually has no target labels but may provide features ${\bm{X}_d}$  to join $ t$'s task of predicting the task label $Y_t$ together. Let use $\mathcal I_d$ to denote its sample IDs.

Hereinafter, we assume the common data sample IDs between the task party and the data parties have already been identified with a data alignment method in any VFL protocol~\cite{Cheng2019SecureBoostAL}, and only these common samples are kept for the VFL task. In other words, we assume all the available data parties share the sample IDs with the task party, and we will concentrate on the essential problem of vertical federated learning.

\begin{definition}[Multi-party VFL]
    Given a task party $t$ with prediction task of $Y_t$, multiple data parties $d\in\bm{\mathcal{D}}$ with sample IDs $\mathcal{I}_d=\mathcal{I}_t=\mathcal{I}$, and a centralized model $\hat{y}_{t[i]} = \mathcal{F}_{CEN}(\bm{x}_{(\{t\}\cup\bm{\mathcal{D}})[i]};\Theta_{CEN})$ trained by aggregating all parties' data with sample ID $i\in\mathcal{I}$, a multi-party VFL task aims to train a model $\hat{y}_{t[i]} = \mathcal{F}_{FED}(\bm{x}_{t[i]}, \bm{x}_{d[i]},\forall d\in\bm{\mathcal{D}}; \Theta_{FED})$ by a decentralized collaborative modelling scheme so that 1) the performance of $\mathcal{F}_{FED}$ is close to that of $\mathcal F_{CEN}$, and 2) each party's raw data will not be accessed by any other parties.
\end{definition}

%\textsc{Definition 3.} \textbf{\textit{A vertical federated learning (VFL) task.}} Given a task party $t$ with its prediction task of $Y_t$, and a number of data parties $ d \in {\bm{\mathcal D}}$, where all the parties share the same sample IDs $\mathcal I_t = {\mathcal I}_d = \mathcal I$,  a centralized model $\hat{y}_{t[i]} =\mathcal F_{CEN}(i|Y_t, \bm X_t, \bm{X}_{\bm{\mathcal D}}, \Theta)$ that could be trained when all parties' data are aggregated, then a VFL task aims to train a model $\hat{y}_{t[i]} =\mathcal F_{FED}(i|Y_t, \bm X_t, \bm{X}_{\bm{\mathcal D}}, \Theta)$ by a carefully designed decentralized collaborative modeling scheme to achieve two goals: 1) each party's raw data will not be accessed by any other parties, and 2) the performance of $\mathcal F_{FED}$ is close to that of $\mathcal F_{CEN}$, where $\Theta$ denotes the parameters, $i\in \mathcal I$ is the sample ID.

\emph{Data valuation} is usually a key phase before launching a multi-party VFL task. From a task party perspective, it can use the valuation to determine whether it is worth inviting other parties and how to price their contributions properly. As to a data party, it regards the pricing to its data as incentives to decide whether to join a VFL task. In this sense, data valuation is considerably important to both task and data parties and their decisions on whether to launch or join a VFL task.

We note that a \textit{task-specific} data valuation method is requisite, as the contribution of a party's data highly relates to specific prediction tasks. %the performance of the model $\mathcal{F}_{FED}$ relates to the task label $Y_t$.
Besides, we usually cannot foreknow the best model for a specific VFL task in its early phase of data valuation for party determination when the parties have not reached an agreement yet on the collaborative modeling; therefore, the VFL model $\mathcal F_{FED}$ would be arbitrary during the data valuation phase, which requires a data valuation method to be \textit{model-free}. 
%a \textit{model-free} data valuation method is often required for party determinations before the collaborative training of $\mathcal F_{FED}$, since we usually cannot foreknow the best model $\mathcal F_{FED}$ for a specific task in such an early stage of VFL. %$\mathcal F_{FED}$ should be arbitrary since we usually cannot foreknow the best model for a specific task, which requires a data valuation method to be \textit{model-free}. 
Finally, a VFL system typically assumes \emph{honest-but-curious} (or equivalently, \emph{semi-honest}) parties~\cite{yang2019federated}; that is, all the parties will follow the predefined mechanism to conduct computations, but try their best to infer other parties' private information with their obtained intermediate computation results. Therefore, we should seek for a secure data valuation method that can keep each data party's raw data unexposed to other parties. With the above considerations, we now formulate our research problem as follows.

%what is the value of the data party $\bar D_j$ in the VFL task of predicting $Y$?

\textbf{Problem Definition (Data Valuation for Multi-party VFL).}~\textit{Given a VFL task with a task party $t$ and multiple data parties $d\in\bm{\mathcal{D}}$, we aim to find a data valuation method for the data parties, which is task-specific, model-free and secure for decentralized data.} 
    
%a task party $t$, a VFL task of predicting $Y_t$, $t$'s data in terms of its features $\bm X_t$ and task label $Y_t$, a set of data parties $d\in \bm{\mathcal{D}}$ who have the same sample IDs as the task party $t$, each data party's feature data ${\bm {X}_d}$, we aim at providing a model-free and task-specific federated data valuation method $\mathcal V(\bm {X}_d;Y_t|\bm X_t, \bm{X}_{\bm{\mathcal D}})$, so that the data value of any party $d \in \bm{\mathcal D}$ in the VFL task of predicting $Y_t$ can be fairly assessed regardless of the model $\mathcal F_{FED}$, and meanwhile the raw data of any party is prevented from being accessed by others.

%\textsc{Definition 4.} \textbf{\textit{Data Valuation Problem for a VFL task.}} 

%In particular, we consider a VFL where a task party $\mathcal T$ holding a set of features $\bm X$  and a target label $Y$. There are also a collection of data parties $\bm {D}$ ($|{\bm {D}}|=l$) who can provide external data to join $u$'s task of predicting $Y$ together. Let use $\bm {\bar X}_i$ to denote the features of each data party $\mathcal D_i \in { \bm{D}}$ $(1\leq i\leq l)$. Then, our problem is how to quantify the value of $\bm {\bar X}_i$ of each data party $\bar u_i$ in predicting $Y$.

%Before devising the method, we highlight the key consideration issues in our design.

%1) \textit{Task-specific} and \textit{Model-free}. First, we clarify that our goal is to . Since the task party can leverage any existing VFL models for prediction, it is desired that the learned data value can be model independently and generally work well for any models.

%2) \textit{No raw data transmission}. To meet the regulation of data privacy, the raw data is restricted to store in each party itself.

%3) \textit{No privacy leakage in intermediate computation}. Besides raw data, to ensure better security, our design does not allow any party to infer other parties' private raw data from the intermediate computation results.

%In this paper, we assume that the common data sample IDs between the task party and the data parties have already been identified with a data alignment method in any VFL protocol~\cite{Cheng2019SecureBoostAL}. Typically, a VFL system also assumes \textit{honest-but-curious} (or called \textit{semi-honest}) parties~\cite{yang2019federated}. The security protection in this paper is also based on the \textit{honest-but-curious} setting. 

%Given this setting, all the parties will follow the predefined mechanism to conduct computations, and try their best to infer other parties' private information with their obtained intermediate computation results. %Besides, our mechanism can also protect all the parties' private information even if \textit{certain parties collude with each other}, which we will elaborate on later.
\vspace{-1em}
\color{black} 

==> VFLValue AIJ/related_work.tex <==
\section{Related Work}

Preserving private information is a fundamental requirement in nowadays' AI applications~\cite{TASSA2021103501,FIORETTO2021103475}. Federate learning (FL) is a privacy-preserving distributed learning paradigm originally proposed by Google~\cite{konevcny2016federated}. After its initial proposal, FL has rapidly attracted a huge amount of attention from both academia and industry \cite{yang2019federated}. Generally speaking, FL conducts collaborative learning with data from multiple parties and meanwhile ensures that no party's data are leaked to any others. According to the data dimension (\emph{i.e.}, feature or sample) that parties collaborate on, FL tasks are categorized into two main classes, \emph{i.e.}, HFL (horizontal FL) and VFL (vertical FL). Specifically, in HFL, parties have different data samples with the same features; while parties usually hold different features of the same data samples in VFL~\cite{yang2019federated}. %In this paper, we focus on the VFL scenario.

Prior FL research efforts are mostly devoted to designing various algorithms in an FL manner. The seminal work \cite{mcmahan2017communication} presents two widely-used HFL learning algorithms, FedSGD and FedAvg, for training neural networks in a federated manner. With FedSGD, HFL parties send every step of gradient descents over local data samples to a server for aggregating models. Comparatively, FedAvg lets each party transmit the average of gradient updates on local data samples for multiple steps to a server for model aggregation. Besides, HFL algorithms are proposed for machine learning models other than neural networks. For instance, a federated matrix factorization algorithm is proposed to achieve a similar performance as the centralized matrix factorization \cite{chai2020secure}; an efficient HFL algorithm is also designed for building boosting decision trees with locality-sensitive hashing \cite{li2020practical}. While VFL is also of significant practical business value \cite{yang2019federated}, it is much under-investigated compared to HFL \cite{wu2020}. %The existing VFL work mostly focus on building various machine learning models.
Cheng et al. \cite{Cheng2019SecureBoostAL} propose the first decision tree algorithm for VFL. The security of the VFL tree is further enhanced by concealing sensitive information of final tree models (e.g., the split thresholds of internal tree nodes) \cite{wu2020}. Hu et al. \cite{hu2019fdml} design an asynchronous stochastic gradient descent algorithm for learning VFL logistic regression and neural network models.

In general, FL algorithms require parties to exchange some insensitive intermediate results (e.g., gradients); however, researchers have found that attackers may still recover raw training data, e.g., images and texts, from gradients \cite{zhu2020deep}. To overcome this pitfall, advanced privacy-preserving computation techniques including homomorphic encryption \cite{aono2017privacy}, secret sharing \cite{Bonawitz2017PracticalSA}, and differential privacy \cite{geyer2017differentially} have been adopted in FL mechanisms. What's more, due to the importance of FL systems in practice, various open-source privacy-preserving FL systems, such as PySyft\footnote{\url{https://github.com/OpenMined/PySyft}}, FedML~\cite{he2020fedml}, FATE\footnote{\url{https://fate.fedai.org/}}, and FedEval~\cite{chai2020fedeval}, have been developed and deployed recently.


In addition to the FL algorithms and systems aforementioned, quantifying the contribution of different parties, i.e., \textit{data valuation}, is another fundamental issue to build a healthy FL ecosystem. With effective data valuation methods, proper incentive mechanisms can then be designed to encourage parties to join the FL community~\cite{yu2020fairness,khan2020federated,cong2020game}. A few prior studies on FL data valuation mainly focus on the HFL scenario \cite{Wei2020,Song2019,Wang2020,liu2020fedcoin}, where the Shapley value~\cite{shapley1953value} is usually adopted in evaluating each party's contribution. Specifically, in a Shapley-value-based HFL valuation framework, each party's value is estimated as the average marginal contribution (i.e., prediction accuracy on a separate test set) to every possible subset of other parties' data samples~\cite{ghorbani2019data}. To address the data valuation problem for the VFL scenario, a pioneering study \cite{Wang2019} suggests using a model-dependent feature importance metric, SHAP \cite{Lundberg2017}, to valuate each party's contribution, which requires a specific training model (e.g., neural networks or SVM). However, data valuation is often a prerequisite before model training for party selection. Our FedValue incorporates a novel model-free valuation metric, Shapley-CMI, and can thus support VFL data valuation before model training. %It is also worth noting that, the work \cite{Wang2019} has not discussed the potential data leakage risks during their valuation process (e.g., model training) ; in comparison, we have carefully analyzed data leakage risks and further propose a secure computation process to alleviate the risks.

How to calculate a joint probability of multiple features from different parties in a privacy-preserving manner is one major challenge of FedValue. Some research approximates such probabilities based on probability distribution assumptions like Gaussian mixture models \cite{Jia2018PrivacyPreservingDJ}. However, these methods will incur obvious approximation errors when the assumption does not hold. Without making any assumptions on the distribution, we leverage MPC (secure Multi-Party Computation) \cite{Bogetoft2009SecureMC} to calculate the multi-feature joint probability via maximum likelihood estimation across parties. Furthermore, we analyze that the key step of the maximum likelihood joint probability estimation is computing the cardinality of the intersection of different parties' data sample ID sets, which is related to the research topic of PSI (Private Set Intersection) in MPC.
%In this work, we focus on server-aided PSI mechanisms, as server-aided ones are verified to be more efficient than non-server ones, and have been widely deployed in practice~\cite{Kamara2014ScalingPS,Le2019TwopartyPS,Bogetoft2009SecureMC}.
Specifically, PSI studies how to obtain intersection elements of multiple sets from different parties in a privacy-preserving manner \cite{freedman2004efficient}, and the state-of-the-art PSI mechanism can support large-scale sets including billions of elements  \cite{Kamara2014ScalingPS}. However, returning intersection elements will still incur VFL parties' data leakage, and thus PSI mechanisms cannot be directly applied for data valuation. More recently, a few studies start exploring the problem of returning a certain function (e.g., cardinality) over PSI, instead of returning the intersection elements. The state-of-the-art work \cite{Le2019TwopartyPS} can compute the intersection cardinality without leaking the intersection elements via secret sharing; however, this protocol~\cite{Le2019TwopartyPS} works for only two parties and cannot support VFL data valuation including more than two parties. Our designed dual-server-aided mechanism overcomes the limitation of party number and can efficiently compute PSI cardinality for an arbitrary number of parties.
\color{black} 
